Variational Diffusion Posterior Sampling with Midpoint Guidance

Diffusion models have recently shown considerable potential in solving Bayesian inverse problems when used as priors. However, sampling from the resulting denoising posterior distributions remains a challenge as it involves intractable terms. To tackle this issue, state-of-the-art approaches formulate the problem as that of sampling from a surrogate diffusion model targeting the posterior and decompose its scores into two terms: the prior score and an intractable guidance term. While the former is replaced by the pre-trained score of the considered diffusion model, the guidance term has to be estimated. In this paper, we propose a novel approach that utilises a decomposition of the transitions which, in contrast to previous methods, allows a trade-off between the complexity of the intractable guidance term and that of the prior transitions. We validate the proposed approach through extensive experiments on linear and nonlinear inverse problems, including challenging cases with latent diffusion models as priors. We then demonstrate its applicability to various modalities and its promising impact on public health by tackling cardiovascular disease diagnosis through the reconstruction of incomplete electrocardiograms. The code is publicly available at \url{https://github.com/yazidjanati/mgps}.

==> appendices/DPS_pitfall.tex <==
\section{Numerical study of DPS-like likelihood approximations}
\label{sec:study_appro\bx _DPS}

We preface this section by an informal discussion on the fact that DPS-like likelihood approximations deteriorates with $k$.


==> appendices/_gaussian_case.tex <==
\section{Gaussian Case}

\subsection*{DDM for Gaussian}
Here, the prior is Gaussian $\prior(\bx _0) = \normpdf (\bx _0; \mu, \sigma^2 \Id)$.
In this case, DDM can be explicitly derived, namely the
\begin{equation}
    \begin{aligned}
        \text{marginals} & \quad
            \fwmarg{k}{}(\bx _k) = \normpdf \big( \bx _k; \sqrt{\acp{k}} \mu, (\var_k + \acp{k} \sigma^2) \Id \big), \\
        \text{denoising densities} & \quad
            \bw{0|k}{\bx _k}{\bx _0} = \normpdf(\bx _0;
                % mean
                \underbrace{\frac{\sqrt{\acp{k}}\sigma^2}{\var_k + \acp{k}\sigma^2} \bx _k + \frac{\var_k}{\var_k + \acp{k}\sigma^2} \mu}_{\mu_{0|k}(\bx _k)},
                % var
                \underbrace{\frac{\var_k \sigma^2}{\var_k + \acp{k}\sigma^2}}_{\sigma_{0|k}^2} \Id)
    \end{aligned}
    \enspace.
\end{equation}
Notice the mean $\mu_{0|k}(\bx _k)$ is linear in $\bx _k$.
Building upon the latter formulas, we derive the expressions of the score and the denoiser
\begin{align}
    s_t(\bx _k) = -\frac{\bx _k - \sqrt{\acp{k}} \mu}{\var_k + \acp{k}\sigma^2}, \quad
    \pE[\bX _0 | \bx _k] = \mu_{0|k}(\bx _k)
    \enspace.
\end{align}


\subsection*{likelihood for linear inverse problems}
The likelihood $\potn{}{}$ defined by a linear inverse problem
\begin{equation}
    y = A \bx _0 + \sigma_y \beps, \quad
    A \in \rset^{d \times d}, \sigma_y > 0, \mathrm{and} \ \beps \sim \normpdf(0, \Id)
    \enspace,
\end{equation}
reads $\potn{}{\bx _0} = \normpdf(y; A \bx _0, \sigma^2 \Id)$.
Under the assumption of Gaussian prior, we can establish the expression of the intermediate likelihoods $\potn{k}{\bx _k}$
\begin{equation}
    \begin{aligned}
        \potn{k}{\bx _k}
            & = \int \potn{}{\bx _0} \bw{0|k}{\bx _k}{\bx _0} \rmd \bx _0 \\
            & = \normpdf(y; A \mu_{0|k}(\bx _k), \sigma_y^2 \Id + \sigma_{0|k}^2 A A^\top)
    \end{aligned}
    \enspace,
\end{equation}
In parallel, the approximate intermediate likelihoods are
\begin{equation}
    \hpotn{k}{\bx _k} = \potn{}{\pE[\bX _0 | \bx _k]} = \normpdf(y; A \mu_{0|k}(\bx _k), \sigma_y^2 \Id)
    \enspace.
\end{equation}
Notice that $\potn{k}{}$ and $\hpotn{k}{}$ differ only in the variance with $\potn{k}{}$ having an extra term in the variance.


\subsection*{Variational approximation}

Learning the mean of the Gaussian variational approximation
\begin{equation}
    \vpibw{\tmid{k}|k+1}{\bx _{k+1}}{\bx _{\tmid{k}}} = \normpdf(\bx _{\tmid{k}}; \varphi, \sigma^2_{\tmid{k}|k+1, 0} \Id)
    \enspace,
\end{equation}
of $\hpibw{\tmid{k}|k+1}{\bx _{k+1}}{\cdot}[]$ reduces to minimizing the following objective function
\begin{equation}
        - \pE[\log \hpotn{\tmid{k}}{\bx _\tmid{k}} ]
        - \pE[\fwtrans{k+1|\tmid{k}}{\bx _{\tmid{k}}}{\bx _{k+1}}]
        - \pE[\log  \fwmarg{\tmid{k}}{}(\bx _{\tmid{k}}) ]
        \enspace,
\end{equation}
where the expected value is taken \wrt \ $\vpibw{\tmid{k}|k+1}{\bx _{k+1}}{\cdot}$.
Since we are not optimizing over the variance, this objective equals up to a constant \wrt \ $\varphi$ to the following
\begin{equation}
    \mathcal{L}_\tmid{k}(\varphi; \bx _{k+1}) =
    \frac{\| y - A \mu_{0|\tmid{k}}(\varphi) \|^2}{2 \sigma_y^2}
    + \frac{ \| \bx _{k+1} -  \sqrt{\frac{\acp{k+1}}{\acp{\tmid{k}}}} \varphi \|^2 }{2 (1 - \frac{\acp{k+1}}{\acp{\tmid{k}}})}
    + \frac{ \| \varphi - \sqrt{\acp{\tmid{k}}} \mu \|^2 }{2 (\var_{\tmid{k}} + \acp{\tmid{k}}\sigma^2)}
    \enspace.
\end{equation}
This objective function is quadratic hence the optimal variational parameter that minimizes it is
\begin{equation}
    \hat{\varphi}(\bx _{k+1}) = -[\nabla_{\varphi}^2 \mathcal{L}_\tmid{k}]^{-1} \nabla_{\varphi} \mathcal{L}_\tmid{k}(0; \bx _{k+1})
    \enspace.
\end{equation}
where $\nabla_{\varphi}^2 \mathcal{L}_\tmid{k}$ is the Hessian and is constant and independent of $\bx _{k+1}$. On the other hand, the gradient depends linearly on $\bx _{k+1}$ and the term in front of it is $\nabla_{\bx _{k+1}} [\nabla_{\varphi} \mathcal{L}_\tmid{k}(0; \bx _{k+1})] =- \frac{ \sqrt{\acp{k+1} / \acp{\tmid{k}}}}{2 (1 - \acp{k+1} / \acp{\tmid{k}})} \Id$.


\subsection*{Mean and covariance of the approximate marginals}

The variational backward is a Gaussian as it is a convolution of two Gaussian distributions
\begin{equation}
    \vpibw{k|k+1}{\bx _{k+1}}{\bx _k} = \int \fwtrans{k|\tmid{k}, k+1}{\bx _\tmid{k}, \bx _{k+1}}{\bx _k} \vpibw{\tmid{k}|k+1}{\bx _{k+1}}{\bx _\tmid{k}} \, \rmd \bx _{\tmid{k}}
    \enspace,
\end{equation}
Knowing that $\fwtrans{k|\tmid{k}, k+1}{\bx _\tmid{k}, \bx _{k+1}}{\bx _k} = \normpdf(\bx _k; a_{k|\tmid{k},k+1} \bx _{k+1} + b_{k|\tmid{k},k+1} \bx _{\tmid{k}}, \sigma^2_{k|\tmid{k},k+1} \Id)$, we have
\begin{equation}
    \begin{aligned}
        \pE[\bX _k | \bx _{k+1}]
            & = a_{k|\tmid{k},k+1} \bx _{k+1} + b_{k|\tmid{k},k+1} \hat{\varphi}(\bx _{k+1}) \\
        \pV[\bX _k | \bx _{k+1}]
            & =  \big( (b_{k|\tmid{k},k+1} \sigma_{\tmid{k}|k+1,0})^2 + \sigma^2_{k|\tmid{k},k+1} \big) \Id
    \end{aligned}
    \enspace,
\end{equation}
where the expected value $\pE$ and variance $\pV$ are taken \wrt \  $\vpibw{k|k+1}{\bx _{k+1}}{\cdot}$.
Marginalizing over $\bX _{k+1} \sim \vpibw{k+1}{}{}$, we obtain the following recursion
\begin{equation}
    \begin{aligned}
        \pE[\bX _k]
            & = a_{k|\tmid{k},k+1} \pE[\bX _{k+1}] + b_{k|\tmid{k},k+1} \hat{\varphi} \big( \pE[\bX _{k+1}] \big), \\
        \pV[\bX _k]
            & = M_{\tmid{k}} \pV[\bX _{k+1}] M_{\tmid{k}}^\top +  \big( (b_{k|\tmid{k},k+1} \sigma_{\tmid{k}|k+1,0})^2 + \sigma^2_{k|\tmid{k},k+1} \big) \Id, \\
        \pE[\bX _n] & = 0,  \pV[\bX _n] = \Id,
    \end{aligned}
\end{equation}
where $M_{\tmid{k}} = a_{k|\tmid{k},k+1} \Id + \frac{ \sqrt{\acp{k+1} / \acp{\tmid{k}}}}{2 (1 - \acp{k+1} / \acp{\tmid{k}})}  b_{k|\tmid{k},k+1} \nabla_{\varphi}^2 \mathcal{L}_\tmid{k}$.

==> appendices/_stale_proofs.tex <==
\section{Proofs}
\label{apdx:proofs}
\subsection{Proof of XXX}
In this section we assume that $\potn{}{\bx} = \normpdf(\obs; Ax, \stdobs^2 \Id)$. We proceed to bound
$$
    \kldivergence{\pibw{\ell|k}{\bx _k}{\cdot}}{\hpibw{\ell|k}{\bx _k}{\cdot}[]} \eqsp.
$$
We have that
\begin{multline*}
    \kldivergence{\pibw{\ell|k}{\bx _k}{\cdot}}{\hpibw{\ell|k}{\bx _k}{\cdot}[]} \\
    = \int \log \frac{\potn{\ell}{\bx _\ell}}{\hpotn{\ell}{\bx _\ell}} \pibw{\ell|k}{\bx _k}{\bx _\ell} \, \rmd \bx _\ell - \log \potn{k}{\bx _k} + \log \int \hpotn{\ell}{\bx _\ell} \bw{\ell|k}{\bx _k}{\bx _\ell} \, \rmd \bx _\ell \eqsp.
\end{multline*}
For the first term, by convexity of $\bx \mapsto \bx \log \bx$ and then definition of $\potn{\ell}{}$, it follows by Jensen's inequality that
\begin{align*}
    \int \log \frac{\potn{\ell}{\bx _\ell}}{\hpotn{\ell}{\bx _\ell}} \pibw{\ell|k}{\bx _k}{\bx _\ell} \, \rmd \bx _\ell & = \int \log \frac{\potn{\ell}{\bx _\ell}}{\hpotn{\ell}{\bx _\ell}} \frac{\potn{\ell}{\bx _\ell} \bw{\ell|k}{\bx _k}{\bx _\ell}}{\potn{k}{\bx _k}} \, \rmd \bx _\ell \\
    & \leq \int \log \frac{\potn{}{\bx _0}}{\hpotn{\ell}{\bx _\ell}} \pibw{0, \ell|k}{\bx _k}{\bx _0, \bx _\ell} \, \rmd \bx _0 \rmd \bx _\ell \eqsp.
\end{align*}
where $\pibw{0, \ell|k}{\bx _k}{\bx _0, \bx _\ell} = \potn{}{\bx _0} \bw{0|\ell}{\bx _\ell}{\bx _0} \bw{\ell|k}{\bx _k}{\bx _\ell} \big/ \potn{k}{\bx _k}$ and is a probability measure.
Next, it holds that
\begin{align}
    \int \log \potn{}{\bx _0} \pibw{0, \ell|k}{\bx _k}{\bx _0} \, \rmd \bx _0 & = - \frac{1}{2 \stdobs^2 }\int \| \obs - A \bx _0 \|^2 \pibw{0|\ell}{\bx _\ell}{\bx _0} \, \rmd \bx _0 \\
    & =
\end{align}
\subsection{Useful computations}
In what follows we assume that $\prior(\bx) = \normpdf(\bx; \zero_\dimx, \Id_\dimx)$ and $\potn{}{\bx} = \normpdf(\obs, A \bx, \stdobs^2 \Id_\dimobs)$. $A \in \rset^{\dimobs \times \dimx}$ is a diagonal rectangular matrix with diagonal $(s_1, \dotsc, s_\dimobs)$. Following \cite[Eq. 2.116]{bishop2006pattern} we have that
$$
    \pi(\bx) = \normpdf(\bx; \Sigma_\obs A^\intercal \obs / \stdobs^2, \Sigma_\obs)
$$
where $\Sigma_\obs = \mathrm{diag}(\var{\obs, 1}, \dotsc, \var{\obs, \dimx})$ where $\var{\obs, i} = \stdobs^2 / (\stdobs^2 + s^2 _i)$ for $\intset{1}{\dimobs}$ and $\var{\obs, i} = 1$ otherwise.

Define $\acp{k| \ell} \eqdef \acp{k} / \acp{\ell}$, $\var{k|\ell} \eqdef 1 - \acp{k|\ell}$. Following the definitions in the main paper we have for all $\ell \in \intset{0}{k-1}$,
$$
   \bw{\ell|k}{\bx _k}{\bx _\ell} = \normpdf(\bx _\ell; \sqrt{\acp{k|\ell}} \bx _k, 1 - \acp{k|\ell}) \eqsp.
$$
Next, the true likelihood $\potn{k}{}$ and approximate DPS likelihood $\hpotn{k}{}$ are defined for all $k \in \intset{0}{n}$ by
\begin{align}
    \potn{k}{\bx _k} & = \normpdf(\obs; \sqrt{\acp{k}} A \bx _k , \Sigma^y _k) \eqsp,\\
    \hpotn{k}{\bx _k} &= \normpdf(\obs; \sqrt{\acp{k}} A \bx _k , \stdobs^2 \Id_\dimobs)
\end{align}
where $\Sigma^y _k = \var{0|k} AA^\intercal + \stdobs^2 \Id_\dimobs$.
Hence, the only difference between the true likelihood and the approximate one lies in the covariance matrix.

Next, for all $\ell, k$ such that $\ell < k$,
\begin{align}
    \hpibw{\ell|k}{\bx _k}{\bx _\ell}[] = \normpdf\big(\bx _\ell;  \mean{\ell|k}^\obs(\bx _k) , \hat\Sigma^\obs _{\ell|k}\big)
\end{align}
where
$$
    \mean{\ell|k}^\obs(\bx _k) \eqdef \hat\Sigma^\obs _{\ell|k} \big\{(\sqrt{\acp{\ell}} / \stdobs^2) A^\intercal \obs+ (\sqrt{\acp{k|\ell}} / \var{k|\ell}) \bx _k\big\}
$$
and $\hat\Sigma^\obs _{\ell|k}$ is a diagonal matrix and $(\hat\Sigma^\obs _{\ell|k})_{i,i} = \frac{\var{k|\ell} \stdobs^2}{\stdobs^2 + s^2 _i \var{k|\ell} \acp{\ell}}$ if $i \leq \dimobs$ and $(\hat\Sigma^\obs _{\ell|k})_{i, i} = \var{k|\ell}$ otherwise. As a result,
$$
    \hpibw{k|k+1}{\bx _{k+1}}{\bx _k}[] = \normpdf\big(\bx _k; \big)
$$
% \begin{proof}[Proof of \Cref{lem:condE_identity}]
%     \label{proof:condE_identity}
%     Define for all $t \in \intset{1}{T}$ and $\bx _t \in \rset^\dimx$
%     $$
%         \post{t}{\bx _t} = \int \fwtrans{t|0}{\bx _0}{\bx _t} \post{}{\rmd \bx _0} \eqsp.
%     $$
%     By \emph{Fisher's identity}, it holds that
%     $$
%         \nabla_{\bx _t} \log \post{t}{\bx _t} = \int \frac{- \bx _t + \sqrt{\acp{t}} \bx _0}{(1 - \acp{t})} \post{0|t}{\rmd \bx _0 | \bx _t} \eqsp,
%     $$
%     and hence,
%     $$
%         \pE_{\post{}{}} [\bX _0 | \bX _t = \bx _t] = \frac{\bx _t + (1 - \acp{t}) \nabla_{\bx _t} \log \post{t}{\bx _t}}{\sqrt{\acp{t}}} \eqsp.
%     $$
%     Next, by noting that
%     $$
%         \post{t}{\bx _t} = \frac{\int \potn{\bx _0} \ }{}
%     $$

% \end{proof}
% \begin{proof}{Proof of XXX}
% \begin{multline*}
%     \kldivergence{\vbwker{0:k-1|k}{\bX _{k}}{\cdot}[\vvparam]}{\abwker{0:k-1|k}{\bX _{k}}{\cdot}}
%     \\
%     = \pE_{\vvparam} \Big[
%         \log \frac{\vbwker{0|k}{\bx _k}{\bx _0}[\vvparam]}{\abwker{0|1}{\bx _1}{\bx _{0}}}
%         + \sum_{j=1}^{k-2} \log \frac{\vbwker{j|j+1,0}{\bx _{j+1}, \bx _0}{\bx _j}[\vvparam]}{\abwker{j|j+1}{\bx _{j+1}}{\bx _{j}}}
%         + \log \frac{\vbwker{k-1|k,0}{\bx _{k}, \bx _0}{\bx _{k-1}}[\vvparam]}{\abwker{k-1|k}{\bx _{k}}{\bx _{k-1}}}
%     \Big]\\
%     = \pE_{\vbwker{0,1|k}{\bx _{k}}{\cdot}[\vvparam]} \big[ \log \frac{\vbwker{0|k}{\bx _k}{\bx _0}[\vvparam]}{\abwker{0|1}{\bx _1}{\bx _{0}}}\big] \\
%         + \sum_{j=1}^{k-2} \pE_{\vbwker{0,j+1|k}{\bx _{k}}{\cdot}[\vvparam]} \big[ \kldivergence{\vbwker{j|j+1,0}{\bx _{j+1}, \bx _0}{\cdot}[\vvparam]}{\abwker{j|j+1}{\bx _{j+1}}{\cdot}} \big] \\
%         + \pE_{\vbwker{0|k}{\bx _{k}}{\cdot}[\vvparam]} \big[ \kldivergence{\vbwker{k-1|k,0}{\bx _{k}, \bx _0}{\cdot}[\vvparam]}{\abwker{k-1|k}{\bx _{k}}{\cdot}} \big]\\
% \end{multline*}

% The $\kldivergence{}{}$ terms have a closed form, hence
% \begin{multline*}
%     \kldivergence{\vbwker{0:k-1|k}{\bX _{k}}{\cdot}[\vvparam]}{\abwker{0:k-1|k}{\bX _{k}}{\cdot}}
%     =  \pE_{\vbwker{0|k}{\bx _{k}}{\cdot}[\vvparam]} \Bigg[\\
%         \log \vbwker{0|k}{\bx _k}{\bx _0}[\vvparam] + \pE_{\vbwker{1|k,0}{\bx _{k}, \bx _0}{\cdot}[\vvparam]} \big[ - \log \abwker{0|1}{\bx _1}{\bx _{0}} \big] \\
%         + \sum_{j=1}^{k-2} \pE_{\vbwker{j+1|k, 0}{\bx _{k}, \bx _0}{\cdot}[\vvparam]} w_j \Big[ \| \bx _0 - \predxs{j+1}(\bx _{j+1}) \|^2 \Big] \\
%         + w_{k-1} \| \bx _0 - \predxs{k}(\bx _{k}) \|^2
%     \Bigg]
% \end{multline*}

% Knowing that we have $-\log \abwker{0|1}{\bx _1}{\bx _{0}} = w_0 \| \bx _0 - \predxs{1}(\bx _{1}) \|^2$ up to an additive constant and that $\vbwker{k|k, 0}{\bx _{k}, \bx _0}{\rmd \bx _k }[\vvparam] = \delta_{\bx _k}(\rmd \bx _k)$, we can simplify the expression
% \begin{multline*}
%     \kldivergence{\vbwker{0:k-1|k}{\bX _{k}}{\cdot}[\vvparam]}{\abwker{0:k-1|k}{\bX _{k}}{\cdot}} = \\
%     H \big( \vbwker{0|k}{\bx _k}{\cdot}[\vvparam] \big) + \sum_{j=0}^{k-1} \pE_{\vbwker{0|k}{\bx _{k}}{\cdot}[\vvparam]} \Bigg[
%         \pE_{\vbwker{j+1|k, 0}{\bx _{k}, \bx _0}{\cdot}[\vvparam]} w_j \Big[ \| \bx _0 - \predxs{j+1}(\bx _{j+1}) \|^2 \Big]
%     \Bigg]
% \end{multline*}

% Since $\vbwker{0|k}{\bx _k}{\cdot}[\vvparam]$ is Gaussian, its entropy can be be evaluated explicitly.
% This gives the final form of the score matching loss
% \begin{multline*}
%     \kldivergence{\vbwker{0:k-1|k}{\bX _{k}}{\cdot}[\vvparam]}{\abwker{0:k-1|k}{\bX _{k}}{\cdot}} = \\
%     \txts \frac{\dimx}{2} \log \big[ \frac{(1 - \acp{k})(\vstd[\vvparam]_0)^2}{1 - \acp{k} + \acp{k} (\vstd[\vvparam]_{0})^2} \big]
%     + \pE_{j, \vbwker{0|k}{\bx _{k}}{\cdot}[\vvparam]} \Bigg[ k w_j
%         \pE_{\vbwker{j+1|k, 0}{\bx _{k}, \bx _0}{\cdot}[\vvparam]} \Big[ \| \bx _0 - \predxs{j+1}(\bx _{j+1}) \|^2 \Big]
%     \Bigg]
% \end{multline*}
% Note that the equality is up to an additive constant independent of $\vvparam$.
% \end{proof}

==> def.tex <==
\def\algo{\sc{VDPS}}
\def\algoname{{\sc{Variational Diffusion Posterior sampler}}}
\def\tauks{L}
\def\PGDM{\Pi \mathrm{GDM}}
\def\DPS{DPS}
\def\imsize{=0.2\hsize}
% \def\eqdef{\ensuremath{:=}}
\def\eqdef{\vcentcolon=}
\def\IP{\mathrm{IP}}
\def\mcgdiff{MCGDiff}
\def\target{\pi}
\def\prior{q}
\def\normconst{\mathcal{Z}}
\def\Idmat{\mathbf{I}}
\def\KL{\mathsf{KL}}
\def\data{Y}
\def\Yspace{\mathsf{Y}}
\def\datadistr{q}
\def\rset{\mathbb{R}}
\def\nset{\mathbb{N}}
\def\rmd{\mathrm{d}}
\def\latent{X}
\def\approxdistr{\operatorname{Q}}
\def\datvar{y}
\def\latvar{x}
\def\eqsp{}
%\def\eqsp{\,}
\def\pV{\mathbb{V}}
\def\pE{\mathbb{E}}
\def\gauss{\mathcal{N}}
\def\N{\mathbb{N}}
\def\Npos{\mathbb{N}_{>0}}
\def\param{\theta}
\def\paramspace{\Theta}
\def\probmeasures{\mathbb{M}_1}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\def\dimobs{{d_\obs}}
\def\dimlatent{p}
\def\Ysigalgebra{\mathcal{Y}}
\def\Xspace{\mathsf{X}}
\def\Xsigalgebra{\mathcal{X}}
\def\variationalfamily{\mathcal{F}}
\def\targetdistr{\pi}
\def\transform{\operatorname{T}}
\def\phispace{\mathsf{T}}
\def\categorical{\mathrm{Categorical}}
\def\1{\mathbbm{1}}
\def\FFBS{\mathrm{FFBS}}
\def\FFBSi{\mathrm{FFBSi}}
\def\PARIS{\mathrm{PaRIS}}
\def\BS{\mathsf{BS}}
\def\bigo{\mathcal{O}}
\newcommandx{\generator}[1][1=]{G^{\genparam _{#1}}}
\def\genparam{\varphi}
\def\pGen{p_\genparam}
\newcommandx{\bwreparam}[1][1=]{\mathcal{G}^{\genparam_{#1}}}
\def\Xset{\mathsf{X}}
\def\Yset{\mathsf{Y}}
\def\sigmaX{\mathcal{X}}
\def\sigmaY{\mathcal{Y}}
\def\1{\mathbbm{1}}
\def\T{\mathrm{\mathbf{T}}}
\def\G{\mathrm{\mathbf{G}}}
\def\pE{\mathbb{E}}
\def\pP{\mathbb{P}}
\def\pV{\mathbb{V}}
\def\N{\mathbb{N}}
\def\plim{\overset{\pP}{\longrightarrow}}
\def\dlim{\Longrightarrow}
\def\gauss{\mathcal{N}}
% \def\cat{\textrm{Cat}}
\def\XX{\mathrm{XX}}
\def\GT{\mathsf{GT}}
\def\BS{\mathsf{BS}}
\def\rmd{\mathrm{d}}
\def\R{\mathbb{R}}
\def\rhs{r.h.s.}
\def\aslim{\overset{a.s.}{\underset{N \to \infty}{\longrightarrow}}}
\def\backsum{\mathcal{T}}
\def\sett{\mathcal{S}}
\def\eve{\mathrm{E}}
\def\Bset{\mathcal{B}}
\def\zero{\mathbf{0}}
\def\bigo{\mathcal{O}}
\def\boldone{\mathbf{1}}
% \def\FFBS{\mathrm{FFBS}}
% \def\FFBSi{\mathrm{FFBSi}}
\def\weightmat{\overline{\mathcal{W}}}
\def\roundW{\mathcal{W}}
\def\simplelim{\underset{N \to \infty}{\lim}}
\def\boundg{G_\infty}
\def\paris{\textit{PaRIS}}
\def\Pbacksum{\widetilde{\backsum}}
\def\bigH{\textbf{H}}
\def\bigF{\textbf{F}}
\def\pos{\mathsf{Pos}}
\def\stdobs{\sigma_\obs}
\def\ft{T}
\def\last{n}
\def\lasto{K}
\def\gvf{\mathcal{G}}
\def\dgvf{\mathcal{G}_\mathrm{D}}
\def\eqinlaw{\smash{\overset{\mathcal{L}}{=}}}
% \def\vmu{\mu^\vparam}
% \def\vstd{\sigma^\vparam}

\newcommand{\stdiobs}[1]{\sigma _{\obs, {#1}}}
\newcommand{\intset}[2]{\llbracket #1, #2 \rrbracket}
\newcommand{\lklhd}[2]{\ifthenelse{\equal{#2}{}}{g^\obs _{#1}}{g^\obs _{#1}(#2)}}
\newcommand{\change}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{\small{#1}}}
\newcommand{\todoo}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{\small{#1}}}
\newcommand{\sylvain}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{\small{\textbf{S} :#1}}}
\newcommand{\jimmy}[1]{\todo[linecolor=magenta,backgroundcolor=magenta!25,bordercolor=magenta]{\tiny{\textbf{JO} : \ #1}}}
\newcommand{\yazid}[1]{\textcolor{blue}{\textbf{YJ}: #1}}
\newcommand{\alain}[1]{\todo[linecolor=cyan,backgroundcolor=cyan!25,bordercolor=cyan]{\small{\textbf{A} :#1}}}
\newcommand{\yohan}[1]{\todo[linecolor=purple,backgroundcolor=purple!25,bordercolor=purple]{\small{\textbf{YP}: #1}}}
\newcommand{\julien}[1]{\todo[linecolor=purple,backgroundcolor=purple!25,bordercolor=purple]{\small{\textbf{J}: #1}}}


\newcommand{\anc}[2]{\smash{A^{#1} _{#2}}}
\newcommand{\yazidd}[1]{\todo[color=blue!20]{{\bf Y:} #1}}
\newcommand{\badr}[1]{\todo[color=red!20]{{\bf B:} #1}}
\newcommand{\divergence}[3]{\mathcal{R}_{#1}(#2 \parallel #3)}
\newcommand{\uweight}[2]{\indx{\widetilde{\omega}}{#1}{#2}}
\newcommand{\weight}[2]{\indx{\omega}{#1}{#2}}
\newcommand{\rnikod}[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand{\flatrnikod}[2]{\rmd #1 / \rmd #2}
\newcommand{\tmidest}[1]{\smash{\target^M _{#1}}}
\newcommand{\SNISest}[1]{\smash{\overline{\target}^M _{#1}}}
\newcommand{\SIRest}[1]{\smash{\widetilde{\target}^M _{#1}}}
\newcommand{\tmiddistr}[4]{\nu^{#1} _{#2}(#4|#3)}
\newcommand{\kldivergence}[2]{\mathsf{KL}(#1 \parallel #2)}
\newcommand{\indx}[3]{#1^{#2} _{#3}}
% \newcommand{\chunk}[3]{#1^{#2:#3}}
\newcommand{\flatchunk}[3]{(\idx{#1}{#2}{}, \dotsc, \idx{#1}{#3}{})}
\newcommand{\Qdistr}[4]{\ifthenelse{\equal{#4}{}}{q^{#1} _{#2}}{q^{#1} _{#2}(#4 |#3)}}
\newcommand{\mudistr}[4]{\ifthenelse{\equal{#4}{}}{\mu^{#1} _{#2}}{\mu^{#1} _{#2}(#4 |#3)}}
\newcommand{\Qpost}[3]{\ifthenelse{\equal{#3}{}}{q^{#1} _{\latent|\data}}{q^{#1} _{\latent|\data}(#3 |#2)}}

\newcommand{\reviewed}[1]{\textcolor{blue}{#1}}
\newcommand{\Const}[1]{\mathcal{C}_{N,b,#1}}
\newcommand{\Gfilt}[2]{\mathcal{G}^N _{#2}}
\newcommand{\proj}[2]{\mathrm{\Pi}_{#1,#2}}
\newcommand{\Gsigma}[2]{\mathcal{G}^{#2}_{#1}}
\newcommand{\card}[1]{\mathrm{Card}(#1)}
\newcommand{\bigprod}[1]{\overline{\Lambda}^{1,2} _{#1}}
\newcommand{\intersect}[2]{\mathrm{I}_{#1}(#2)}
\newcommand{\joint}[1]{\gamma _{#1}}
\newcommand{\pred}[1]{\eta _{#1}}
\newcommandx{\predx}[3][2=0,3=\param]{\hat{x}^{#3} _{#2|#1}}
\newcommandx{\bwmean}[1]{m_{#1}}
\newcommandx{\bwvar}[1]{\sigma_{#1}}
\newcommandx{\predxs}[3][2=0,3=\optparam]{\hat{x}^{#3} _{#2|#1}}
\newcommandx{\prednoise}[2][2=\param]{\smash{\hat{\epsilon}^{#2} _{#1}}}
% \newcommand{\filter}[1]{\phi _{#1}}
\newcommand{\F}[1]{\mathcal{F}^N _{#1}}
\newcommand{\GG}[1]{\mathrm{\mathbf{G}}_{#1}}
\def\forward{\mathrm{f}}
\def\backward{\mathrm{b}}
\def\L{\mathrm{\mathbf{L}}}
\newcommand{\smooth}[2]{\phi_{#1 | #2}}
\newcommand{\smoothN}[3]{\phi^{#3} _{#1 | #2}}
\newcommand{\particletraj}[2]{\xi^{#1 _{0:#2}} _{0:#2}}
\newcommand{\particlecloud}[1]{\bm \xi^{1:N} _{0:#1}}
\newcommand{\bwker}[1]{\mathrm{\mathbf{B}} _{\phi_{#1}}}
\newcommand{\bwpath}[1]{\mathrm{\mathbf{T}} _{#1}}
\newcommand{\transition}[1]{\ifthenelse{\equal{#1}{0}}{M_0}{M_{#1}}}
\newcommand{\fakeprior}{\gamma}
\newcommand{\Q}[1]{\mathrm{\mathbf{Q}}_{#1}}
\newcommand{\Qmarg}[1]{\overline{\mathrm{\mathbf{Q}}}_{#1}}
\newcommand{\asymptvarest}[2]{\ifthenelse{\equal{#2}{}}{\ensuremath{\Gamma _{0: #1 \mid #1}}}{\ensuremath{\Gamma^{#2}_{0: #1 \mid #1}}}}
\newcommand{\asymptvarffbs}[2]{\ifthenelse{\equal{#2}{}}{\ensuremath{\Gamma^{\textrm{FFBS}} _{0: #1 \mid #1}}}{\ensuremath{\Gamma^{#2, \textrm{FFBS}}_{0: #1 \mid #1}}}}
\newcommand{\transitiondens}[1]{\ifthenelse{\equal{#1}{0}}{m_0}{m_{#1}}}
\newcommand{\bitransition}[2]{\mathcal{M}^{#1} _{#2}}
\newcommand{\mumeasure}[1]{\mathcal{Q}_{#1}}
\newcommand{\bounded}[1]{\ifthenelse{\equal{#1}{}}{\ensuremath{\mathsf{F} (\mathcal{X})}}{\ensuremath{\mathsf{F} (\mathcal{X}^{\otimes {#1}})}}}
\newcommand{\measurable}[1]{\ifthenelse{\equal{#1}{}}{\ensuremath{\mathsf{F}(\mathcal{X})}}{\ensuremath{\mathsf{F}(\mathcal{X}^{\otimes {#1}})}}}
\newcommand{\additive}[1]{\mathbb{A}_b(\mathcal{X}^{\otimes #1})}
\newcommand{\muest}[2]{\mathcal{Q}^{N,#1} _{#2}}
\newcommand{\backwardTest}[4]{\mathrm{\mathbf{T}}^{#1} _{#2}(#3, #4)}
\newcommand{\backwardT}[3]{\mathrm{\mathbf{T}}_{#1}(#2, #3)}
\newcommand{\predasymptvar}[2]{\mathcal{V}^{\infty}_{\eta, #1} \left(#2\right)}
\newcommand{\jointasymptvar}[2]{\mathcal{V}^{\infty}_{\gamma, #1} (#2)}
\newcommand{\jointasymptvarestim}[2]{\mathcal{V}^{N}_{\gamma, #1} (#2)}
\newcommand{\predasymptvarestim}[2]{\mathcal{V}^{N}_{\eta, #1} (#2)}
\newcommand{\asymptvar}[1]{\mathcal{V}^{\infty} _{#1}}
\newcommand{\asymptvarestim}[2]{\mathcal{V}^{N,#2} _{#1}}
\newcommand{\scdjointasymptvarestim}[2]{\overline{\mathcal{V}}^{N}_{\gamma,#1} (#2)}
\newcommand{\jointestimchan}[2]{\mathcal{V}^{N, \infty}_{#1} (#2)}
\newcommand{\jointestimlee}[2]{\mathcal{V}^{N, \infty}_{#1} (#2)}
\newcommand{\idealasymptvarest}[2]{\Gamma^{#2} _{#1} (h_{0:#1})}
\newcommand{\jointvarestim}[3]{\mathcal{V}^{N, #3}_{\gamma, #1} (#2)}
\newcommand{\tbtasymptvarestim}[2]{\mathcal{\overline{V}}{\vphantom{\mathcal{V}}}^{N,#2} _{#1}}
\newcommand{\scdjointvarestim}[3]{\overline{\mathcal{V}}^{N, #3}_{\gamma, #1} (#2)}
\newcommand{\parisasymptvar}[2]{\mathsf{V}^{N,M} _{#1}}
\newcommand{\asymptvaresttf}[2]{\ensuremath{\widetilde{\Gamma}^{#2} _{#1} (h_{0:#1})}}
% \newcommand{\esssup}[2][]
% {\ifthenelse{\equal{#1}{}}{\left\| #2 \right\|_\infty}{\left\| #2 \right\|^2_{\infty}}}
% \newcommand{\eqdef}{\ensuremath{:=}}
% \newcommand{\eqsp}{}
% \newcommand{\weight}[2]{\tilde{\omega}^{#1} _{#2}}
% \newcommand{\normweight}[2]{\mathcal{W}^{#1} _{#2}}
\newcommand{\normweight}[2]{\omega^{#1} _{#2}}
\newcommand{\particle}[2]{\xi^{#1} _{#2}}
\newcommand{\particleQ}[2]{\mathsf{Q}^N _{#2}(A^{1:N} _{#1}, \rmd \particle{1:N}{#2})}
\newcommand{\condparticleQ}[3]{\mathsf{Q}^{#3, N} _{#1 + 1}(#2 _{#1 + 1};  \rmd \particle{1:N \setminus \{#2 _{#1 + 1}\}}{#1 +1}, A^{1:N} _{#1})}
\newcommand{\smclaw}[1]{\mathrm{P}^N (A^{1:N} _{0:#1-1},\rmd \particle{1:N}{0:#1})}
\newcommand{\condsmclaw}[3]{\mathrm{P}^N _{#3} (#2 _{0:#1};  A^{1:N} _{0:#1 -1},\rmd \particle{1:N \setminus \{#2 _{0:#1}\}}{0:#1})}
\newcommand{\condchi}[1]{\bar{\chi}(#1 _{0}; \rmd \particle{1:N \setminus \{ #1 _0\}}{0})}
\newcommand{\smclawtraj}[2]{\mathrm{P}^N (\rmd \particle{}{0:#1}, A _{0:#1-1}, #2 _{0:#1})}
% \newcommand{\mixture}[3]{
%     \ifthenelse{\equal{#3}{}}{\mathrm{Q} _{#1}(\particle{1:N}{#1 -1}, \rmd \particle{#2}{#1})}{\mathrm{Q}^{\otimes #3} _{#1}(\particle{1:N}{#1}, \rmd \particle{#2}{#1})}}
\newcommand{\ffbsasymptvar}[3]{\mathcal{V}^{#1} _{#2 | #3}}
\newcommand{\parismuest}[2]{\widetilde{\mathcal{Q}}^{N,M} _{#2}}
% \newcommand{\A}[2]{\ifthenelse{\equal{#2}{}}{(\mathbf{A}{\mathbf{\ref{#1})}}}{(\mathbf{A}\mathbf{\ref{#1}:\ref{#2}})}}
\newcommand{\As}[2]{\ifthenelse{\equal{#2}{}}{(\mathbf{A}{\mathbf{\ref*{#1})}}}{(\mathbf{A}\mathbf{\ref*{#1}:\ref*{#2}})}}
\newcommand{\RQ}[1]{(\textbf{Q}{#1})}
\newcommand{\muDDIM}[1]{\mu_{#1}}

%NEO def

\def\param{\theta}
\def\gauss{\Normal}
 \def\elboneq{\mathcal{L}_{\IFIS}}
\def\argmax{\arg \max}
\def\hparam{\theta^*}
\def\Param{\Theta}
\def\logit{\operatorname{logit}}
 \def\flow{\mathbf{T}}
\def\Cat{\operatorname{Cat}}
\def\tU{\tilde{U}}
 \def\mass{\mathrm{M}}
 \def\Normal{\mathrm{N}}
  \providecommand{\assumptionname}{Assumption}
  \providecommand{\corollaryname}{Corollary}
  \providecommand{\lemmaname}{Lemma}
  \providecommand{\propositionname}{Proposition}
  \providecommand{\remarkname}{Remark}
\providecommand{\theoremname}{Theorem}
%\usepackage[disable]{todonotes}

\def\plaw{\operatorname{g}}

\def\simiid{\overset{\operatorname{iid}}{\sim}}
%% math commands go here
\def\IFIS{\ensuremath{\operatorname{NEO}}}
\def\InFiNE{{\small \IFIS}}
\def\NEO{{\small \IFIS}}

\def\MC{\mathrm{MC}}
\def\transfo{\operatorname{T}}
\def\dmid{\left.\middle\|\right.}
\def\rmd{\operatorname{d}\hspace{-2pt}}
\def\Id{\mathbf{Id}}
\def\PP{\mathbb{P}}
\def\QQ{\mathbb{Q}}
% \def\pE{\mathbb{E}}
\def\PVar{\mathrm{Var}}
\def\mcf{\mathcal{F}}
\def\Ind{\mathbb{I}}
\def\ELBO{\operatorname{ELBO}}
\def\rset{\mathbb{R}}
\def\brset{\overline{\mathbb{R}}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}_{>0}}
\def\Ber{\mathrm{Ber}}
\def\dummy{f}
\def\nmeasrho{\tilde{\measrho}}
\def\suppvarpi{\mathbb{S}}
\newcommandx{\Exp}[2][1=]{\ensuremath{\pE_{#1}\left[ #2\right]}}
\def\Var{\operatorname{Var}}
\newcommandx{\marginal}[2][1=]{\ensuremath{\xi^{#2}_{#1}}}

\newcommandx{\margindensm}[2]{m_{#1}^{#2}}
\newcommandx{\margindensmu}[4]{m_{#1}^{#2}(#3|#4)}
\newcommand{\partint}[1]{ \left \lfloor #1 \right \rfloor}

\newcommandx{\margindens}[4][4=]{\ifthenelse{\equal{#3}{}}{q_{#1}^{#4}(#2)}{q_{#1,#3}^{#4}(#2)}}
\newcommandx{\margindensw}[3][3=]{\ifthenelse{\equal{#3}{}}{q_{#1}^{#2}}{q_{#1,#3}^{#2}}}
\newcommand{\Mtrans}[4]{Q_{#1,#4}(#2,#3)}
\newcommand{\Mtransw}[2]{Q_{#1,#2}}
% \newcommand{\chunk}[3]{#1_{#2:#3}}
% \newcommand{\KL}[2]{\operatorname{KL}\left(#1\Vert #2\right)}
\newcommand{\KLLigne}[2]{\operatorname{KL}(#1| #2)}
\def\lowerbound{\mathcal{L}}
\def\lowerboundaux{\mathcal{L}_{\mathrm{aux}}}
\def\tlowerboundaux{\tilde{\mathcal{L}}_{\mathrm{aux}}}
\def\rmd{\mathrm{d}}
\def\bigO{\mathcal{O}}
\def\eqsp{\,}

\def\fwdtransfo{T}
\newcommandx{\fwdtransfoparam}[2]{\fwdtransfo_{#1,#2}}
\def\famtransfo{\mathcal{T}}
\def\invtransfo{\mathring{\fwdtransfo}}
\def\trueflow{\mathsf{T}}

\def\dmhratio{\mathring{\alpha}_{\phi,\tu}}
\def\counting{\mathsf{c}}
% \renewcommand{\sqrt}[1]{#1 ^{1/2}}
\def\msa{\mathsf{A}}
% \def\borel{\mathcal{B}}
\newcommand{\defeq}{\vcentcolon=}
% \newcommand{\eqdef}{=\vcentcolon}

\def\dimE{M}
\def\dimS{D}


\def\eg{\text{e.g.}}



\def\rmb{\mathrm{b}}

\def\mcu{\mathcal{U}}
\def\wrt{w.r.t.}

\def\phibf{\pmb{\phi}}
\def\bfphi{\phibf}

% Operands
\newcommand{\absolute}[1]{\left\vert #1 \right\vert}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\absLigne}[1]{\vert #1 \vert}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathsf{TV}}}
\newcommand{\tvnormEq}[1]{\left \| #1 \right \|_{\mathrm{TV}}}
\newcommandx{\Vnorm}[2][1=V]{\| #2 \|_{#1}}
\newcommandx{\VnormEq}[2][1=V]{\ensuremath{\left\| #2 \right\|_{#1}}}
% \newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
% \newcommandx{\normLigne}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2\Vert^{#1}}}
\newcommand{\crochet}[1]{\left\langle#1 \right\rangle}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\newcommand{\parentheseLigne}[1]{(#1 )}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\newcommand{\parentheseDeuxLigne}[1]{[ #1 ]}
\newcommand{\defEns}[1]{\left\lbrace #1 \right\rbrace }
\newcommand{\defEnsLigne}[1]{\lbrace #1 \rbrace }
\newcommand{\defEnsPoint}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsPointDeux}[1]{\left. #1 \right  \rbrace }
\newcommand{\defEnsL}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsR}[1]{\left. #1 \right  \rbrace }

%\newcommand{\defSystem}[1]{\left\lbrace #1 \right. }

\newcommand{\ps}[2]{\left\langle#1,#2 \right\rangle}
\newcommand{\psLigne}[2]{\langle#1,#2 \rangle}

% Relations
\newcommand{\divid}{\mid}
\newcommand{\ndivide}{\nmid}

% Proba
\newcommand{\proba}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\probaCond}[2]{\mathbb{P}\left( \left. #1  \middle\vert #2 \right.\right)}
\newcommand{\probaLigne}[1]{\mathbb{P}( #1 )}
\newcommandx\probaMarkovTilde[2][2=]
{\ifthenelse{\equal{#2}{}}{{\widetilde{\mathbb{P}}_{#1}}}{\widetilde{\mathbb{P}}_{#1}\left[ #2\right]}}
\newcommand{\probaMarkov}[2]{\mathbb{P}_{#1}\left[ #2\right]}
\newcommand{\expe}[1]{\pE \left[ #1 \right]}
\newcommand{\expeExpo}[2]{\pE^{#1} \left[ #2 \right]}
\newcommand{\expeLigne}[1]{\pE [ #1 ]}
\newcommand{\expeLine}[1]{\pE [ #1 ]}
\newcommand{\expeMarkov}[2]{\pE_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovLigne}[2]{\pE_{#1} [ #2 ]}
\newcommand{\expeMarkovExpo}[3]{\pE_{#1}^{#2} \left[ #3 \right]}
\newcommand{\probaMarkovTildeDeux}[2]{\widetilde{\mathbb{P}}_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovTilde}[2]{\widetilde{\pE}_{#1} \left[ #2 \right]}
\newcommand{\tmestep}[1]{{t_{#1}}}
% Environments

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}



%fleche limite
\newcommand{\flecheLimite}{\underset{n\to+\infty}{\longrightarrow}}
\newcommand{\flecheLimiteOption}[2]{\underset{#1\to#2}{\longrightarrow}}
\newcommand{\flecheLimiteHaut}{\overset{n\to+\infty}{\longrightarrow}}


%notation infini
\newcommand{\plusinfty}{+\infty}

%notation egale
\newcommand{\egale}[1]{\ensuremath{\underset{#1}{=}}}

%plusieurs ligne indice
%\sum\limits_{\substack{i=0 \\ i \neq i_0}}^{n}{A_



\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


\newcommand{\hilbert}{\mathcal{H}}


\def\ie{\textit{i.e.}}
%\def\as{almost surely}
\def\cadlag{càdlàg}
\def\eqsp{\;}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}
\renewcommand{\iint}[2]{\left\lbrace #1,\ldots,#2\right\rbrace}
\newcommand{\iintLigne}[2]{\lbrace #1,\ldots,#2\rbrace}


\def\primr{f_r}
\def\primrO{f_{r_0}}



% \newcommand{\1}{\mathbbm{1}}
% \newcommand{\indi}[1]{\1_{#1}}
\newcommand{\indiacc}[1]{\mathbbm{1}_{\{ #1   \}}}
% \newcommandx{\weight}[2][2=n]{\omega_{#1,#2}^N}
\newcommand{\loi}{\mathcal{L}}
\newcommand{\boule}[2]{\operatorname{B}(#1,#2)}
\newcommand{\ball}[2]{\operatorname{B}(#1,#2)}
\newcommand{\boulefermee}[2]{\overline{\mathrm{B}}(#1,#2)}
\newcommand{\diameter}{\operatorname{diam}}
\newcommand{\deta}{d_{\eta}}
% \def\divergence{\operatorname{div}}
\def\TV{\mathrm{TV}}
\def\Tvarpi{T_\varpi}
\newcommand{\tme}[1]{{t_{#1}}}
% \def\argmax{ \arg \max}
% \def\argmin{ \arg \min}



 \newcommand{\alaini}[1]{\todo[color=black!20,inline]{{\bf AD:} #1}}
%   \newcommand{\alain}[1]{\todo[color=black!20]{{\bf AD:} #1}}
% \newcommand{\tcb}[1]{\textcolor{blue}{#1}}
 \newcommand{\eric}[1]{\todo[color=red!20]{{\bf Eric:} #1}}
  \newcommand{\xian}[1]{\todo[color=orange!30]{{\bf Xian:} #1}}
  \newcommand{\achille}[1]{\todo[color=blue!30]{{\bf AT:} #1}}

\def\as{almost surely}
\def\dist{\operatorname{dist}}

\newcommand{\seq}[3]{(#1) _{#2} ^{#3}}
\newcommandx\sequence[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2}, \eqsp #2 \in #3 \}}}}
\newcommandx\sequenceD[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{( #1)_{ #2 \in #3} }}}

\newcommandx{\sequencen}[2][2=n\in\N]{\ensuremath{\{ #1_n, \eqsp #2 \}}}
\newcommandx\sequenceDouble[4][3=,4=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ (#1_{#3},#2_{#3}) \}}}{\ensuremath{\{  (#1_{#3},#2_{#3}), \eqsp #3 \in #4 \}}}}
\newcommandx{\sequencenDouble}[3][3=n\in\N]{\ensuremath{\{ (#1_{n},#2_{n}), \eqsp #3 \}}}


\def\iid{i.i.d.}
\def\ifof{if and only if}
% \def\eg{e.g.}




\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}


\def\momentNoise{\mathrm{m}}
\def\bfe{\mathbf{e}}

\def\bfv{\mathbf{v}}
\def\ebf{\mathbf{e}}
\def\vbf{\mathbf{v}}


\def\Id{\operatorname{Id}}

\def\tildetheta{\tilde{\theta}}

\def\calC{\mathcal{C}}

\def\varphibf{\operatorname{g}}
\newcommandx{\CPE}[3][1=]{{\mathbb E}_{#1}\left[\left. #2 \middle \vert #3 \right. \right]} %%%% esperance conditionnelle
\newcommandx{\CPVar}[3][1=]{\mathrm{Var}^{#3}_{#1}\left\{ #2 \right\}}
\newcommand{\CPP}[3][]
{\ifthenelse{\equal{#1}{}}{{\mathbb P}\left(\left. #2 \, \right| #3 \right)}{{\mathbb P}_{#1}\left(\left. #2 \, \right | #3 \right)}}

\def\Ascr{\mathscr{A}}
\def\scrA{\mathscr{A}}
\def\scrB{\mcbb}
\def\scrC{\mathscr{C}}

\def\barL{\bar{L}}

\def\YL{\mathbf{Y}}
\def\XEM{X}
\def\steps{\gamma}
\def\measSet{\mathbb{M}}

\newcommand\Ent[2]{\mathrm{Ent}_{#1}\left(#2\right)}
\newcommandx{\osc}[2][1=]{\mathrm{osc}_{#1}(#2)}

\def\Ybar{\bar{Y}}
\def\Id{\operatorname{Id}}
\def\IdM{\operatorname{I}_d}
\newcommand\EntDeux[2]{\Ent_{#1}\left[#2 \right]}
\def\Ltwo{\mathrm{L}^2}
\def\Lone{\mathrm{L}^1}
\newcommand\densityPi[1]{\frac{\rmd #1}{\rmd \pi}}
\newcommand\densityPiLigne[1]{\rmd #1 /\rmd \pi}
\newcommand\density[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand\densityLigne[2]{\rmd #1/\rmd #2}

\def\V{V}
\def\VD{V}
\def\Vsp{V^{\sphere^d}_{\b,\beta}}
\def\Vr{V^{\rset^d}_{\b,\c,\beta}}

\def\Prset{P^{\rset^d}}
\def\Psphere{P^{\sphere^d}}

\def\n{\mathrm{n}}
\def\Vpsi{\psi}
\def\Vkappa{\kappa}
\def\Vkappat{\tilde{\kappa}}
\def\Vchi{\chi}
\def\Vchit{\tilde{\chi}}
\def\Vphi{\phi}
\def\Vrho{\rho}
\def\psiV{\Vpsi}
\def\rhoV{\Vrho}
\def\phiV{\Vphi}
\def\fV{f}
\def\Vf{\fV}
\def\kappaVt{\tilde{\Vkappa}}
\def\kappaV{\Vkappa}
\def\chiV{\Vchi}
\def\chiVt{\Vchit}


\def\a{a}
\def\b{b}
\def\c{c}
\def\e{e}
\def\rU{\mathrm{r}}

\def\domain{\mathrm{D}}

\def\martfg{M^{f,g}}
\newcommand\Ddir[1]{D_{#1}}
\newcommand\maxplus[1]{\parenthese{#1}_+}
\def\Refl{\mathrm{R}}
\def\phibf{\pmb{\phi}}
\def\Gammabf{\mathbf{\Gamma}}


%\def\transpose{\operatorname{T}}
\def\transpose{\intercal}
\def\v{v}
\def\w{w}
\def\y{y}
\def\z{z}
%%%% bar

\def\bb{\bar{b}}
\def\bgamma{\bar{\gamma}}
\def\bU{\bar{U}}
\def\Ub{\bU}
\def\lambdab{\bar{\lambda}}
\def\blambdab{\bar{\lambda}}
\def\bv{\bar{v}}
\def\vb{\bv}
\def\yb{\bar{y}}
\def\by{\yb}
\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\taub{\bar{\tau}}

\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}

\def\pib{\bar{\pi}}
\def\bpi{\pib}

\def\S{S}
\def\target{\pi}
\def\proposal{\rho}
\def\weightfunc{\tilde{w}}
\newcommand{\chunku}[3]{#1^{#2:#3}}
\newcommand{\chunkl}[3]{#1_{#2:#3}}
\newcommand{\chunkul}[5]{#1_{#2:#3}^{#4:#5}}
\newcommand{\chunkum}[4]{#1^{#2:#3 \setminus \{#4\}}}
\newcommand{\chunkulm}[6]{#1_{#2:#3}^{#4:#5 \setminus \{#4\}}}
\def\tmidIR{\ensuremath{\operatorname{i-SIR}}}
%%%%
% \tilde

\def\tr{\tilde{r}}
\def\tc{\tilde{c}}
\def\tmsk{\tilde{\msk}}
\def\tW{\tilde{W}}
\def\tvarsigma{\tilde{\varsigma}}
% \def\tv{\tilde{v}}
\def\vt{\tv}
\def\yt{\tilde{y}}
\def\ty{\yt}
\def\Mt{\tilde{M}}
\def\tM{\Mt}

\def\tx{\tilde{x}}
\def\xt{\tx}
\def\Xt{\tilde{X}}
\def\Yt{\tilde{Y}}
\def\Gt{\tilde{G}}
\def\Et{\tilde{E}}
\def\Tt{\tilde{T}}
\def\St{\tilde{S}}
\def\taut{\tilde{\tau}}

\def\tX{\tilde{X}}
\def\tY{\tilde{Y}}
\def\tG{\tilde{G}}
\def\tE{\tilde{E}}
\def\tT{\tilde{T}}
\def\tS{\tilde{S}}
\def\ttau{\tilde{\tau}}
\def\teta{\tilde{\eta}}
\newcommand{\ttheta}{\tilde{\theta}}


%%%%%
% \bar
\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\Sb{\bar{S}}
\def\taub{\bar{\tau}}
\def\Hb{\bar{H}}
\def\Nb{\bar{N}}


\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}
\def\bS{\bar{S}}
\def\bH{\bar{H}}
\def\bN{\bar{N}}

%%%%%%%%

\def\mgU{\mathrm{m}_{\nabla U}}
\def\MintDrift{I}
\def\CU{C_U}
\def\RU{R_1}
\def\RV{R}
\def\Reps{R_{\epsilon}}
\def\Resp{\Reps}
\def\veps{\varepsilon}
\def\sphere{\mss}

%\def\suppvarpi{\zset}
\def\bound{M_{\transfo}^{\varpi}}
\def\nablaUt{\overline{\nabla U}}
\def\measureSphere{\nu^d}
\def\wcont{w_t^\mathrm{c}}
\def\etaU{\eta}
\def\epsilonU{\epsilon}
\def\rhoTcont{\rhoT^{\operatorname{c}}}
\def\NEIS{\ensuremath{\operatorname{NEIS}}}
\def\Jac{\mathbf{J}}
\newcommand{\JacOp}[1]{\Jac_{#1}}
\def\jac{\operatorname{Jac}}
\def\sign{\operatorname{sign}}
\def\rate{\lambda_{\mathrm{r}}}
\newcommand{\intentier}[2]{[#1:#2]}
\newcommand{\intentierU}[1]{[#1]}
%\newcommand{\intentier}[2]{#1:#2}
\def\measrho{\boldsymbol{\rho}}
\def\rmi{\mathrm{I}}
\def\ne{\mathrm{ne}}
\def\const{\operatorname{Z}}
\def\estConst{\widehat{\const}^{\varpi}}
\newcommand{\estConstC}[1]{\widehat{\const}^{\varpi}_{#1}}
\newcommand{\estConstCphi}[2]{\widehat{\const}_{#1}^{#2}}
\newcommand{\hatpi}[1]{\hat{\pi}_{#1}}
%\def\hatpi{\hat{\pi}}
\def\measpi{\boldsymbol{\pi}}
\def\measprop{\boldsymbol{\rho}}
\def\measq{\boldsymbol{q}}

\def\trace{\operatorname{tr}}
\def\sigmaS{\sigma^2}
\def\adj{\operatorname{adj}}
\newcommand{\ensemble}[2]{\left\{#1\,:\eqsp #2\right\}}
\newcommand{\ensembleLigne}[2]{\{#1\,:\eqsp #2\}}
\newcommand{\set}[2]{\ensemble{#1}{#2}}

\def\rmD{\mathrm{D}}%%rmd déjà pris
\def\mrd{\mathrm{D}}
\def\mrc{\mathrm{C}}

% \def\diag{\Delta_{\rset^d}}

\def\lyap{V}
\newcommand\coupling[2]{\Gamma(\mu,\nu)}
\def\supp{\mathrm{supp}}
\def\tpi{\tilde{\pi}}
\def\tPi{\tilde{\Pi}}
\newcommand\adh[1]{\overline{#1}}

\def\ACb{\mathrm{AC}_{\mathrm{b}}}

\def\opK{\mathrm{K}}

\newcommand{\fracm}[2]{\left. #1 \middle / #2 \right.}

\newcommand{\complementary}{\mathrm{c}}

\def\poty{H}
\def\diam{\mathrm{diam}}
\def\talpha{\tilde{\alpha}}
\def\Leb{\mathrm{Leb}}
\newcommand{\iintD}[2]{\{#1,\ldots,#2\}}
\def\interior{\mathrm{int}}
\def\iff{ if and only if }

\def\vareps{\varepsilon}
\def\varespilon{\varepsilon}
\def\si{\text{ if } }
\def\projd{\operatorname{proj}^{\msd}}
\def\Phibf{\mathbf{\Phi}}

\def\RKer{R_{\gamma}}

\def\VEa{V}
\def\KUa{K}
\def\vol{\operatorname{Vol}}

\newcommand*\Let[1]{\State #1 }

\def\mU{\mathrm{m}}

\newcommand\fraca[2]{(#1)/(#2)}

\def\ccur{\mathtt{c}}
\def\Ve{V_{\rme}}
\def\Rad{\operatorname{Rad}}
%%% mathsf
\def\msi{\mathsf{I}}
\def\msw{\mathsf{W}}
\def\msa{\mathsf{A}}
\def\msd{\mathsf{D}}
\def\msk{\mathsf{K}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\msat{\tilde{\mathsf{A}}}
\def\msb{\mathsf{B}}
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{O}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\tmsu{{\mathsf{U}}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
\def\msx{\mathsf{X}}
\def\msy{\mathsf{Y}}

\def\msphi{\mathsf{\Phi}}

%% mathcal
\def\mca{\mathcal{A}}
\def\mcl{\mathcal{L}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcbb{\mathcal{B}}  %%% \mcb est déjà pris
\def\mcc{\mathcal{C}}
\def\mcy{\mathcal{Y}}
\def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}

%% mathbb

\def\rset{\mathbb{R}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^*}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}


%%%% mathrm


\def\rmP{\mathrm{P}}
\def\rmQ{\mathrm{Q}}
\def\rml{\mathrm{L}}
\def\rmR{\mathrm{R}}
\def\rmS{\mathrm{S}}
\def\rmT{\mathrm{T}}
\def\rmM{\mathrm{M}}
\def\Prm{\mathrm{P}}
\def\rmb{\mathrm{b}}
\def\mrb{\mathrm{b}}
\def\rmd{\mathrm{d}}
\def\rmZ{\mathrm{Z}}
\def\mrd{\mathrm{d}}
\def\mre{\mathrm{e}}
\def\rme{\mathrm{e}}
\def\rmn{\mathrm{n}}
\def\mrn{\mathrm{n}}
\def\mrc{\mathrm{C}}
\def\mrcc{\mathrm{c}}
\def\rmc{\mathrm{C}}
\def\rmcc{\mathrm{c}}
\def\rma{\mathrm{a}}
\def\mra{\mathrm{a}}
\def\rmC{\mathrm{C}}

\def\tu{u}
\def\FamilyVar{\mathcal{Q}}
\def\RWM{\scriptscriptstyle{\operatorname{RWM}}}
\def\MALA{{\scriptscriptstyle{\operatorname{MALA}}}}
\def\MH{\mathsf{MH}}
\def\stephmc{\upgamma}
\def\Sigmahmc{\Sigma}
\def\densgauss{\varphibf}
\def\LF{\mathsf{LF}}
\def\Refresh{\mathsf{ref}}

% \newcommand{\card}[1]{\vert #1\vert}
\def\tz{\tilde{z}}

\def\Idd{\mathrm{Id}}
\def\likeratio{\kappa}
\def\minor{\varepsilon}

\newcommandx{\estpiNaive}[3][1=g,2=N,3=f]{\hat{\pi}_{#1}^{#2}(#3)}
\def\bmeaspi{\bar{\measpi}}
\def\bmeasq{\bar{\measq}}

\def\rhobf{\measrho}

\def\bfm{\mathbf{m}}

\newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
\newcommandx{\normLigne}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2 \Vert^{#1}}}
\def\gaussianD{\operatorname{g}}
\def\rhoT{\rho_{\transfo}}
\def\constT{\const_{\transfo}}
\def\pdf{p.d.f.}
% \def\wrt{with respect to}

\def\oQ{\operatorname{Q}}
\def\oP{\operatorname{P}}


\def\infineIS{I^{\NEO}_{\varpi,N}}
\def\infineISh{I^{\NEO}_{\varpi,N,h}}
\def\infineSNIS{J^{\NEO}_{\varpi,N}}
\def\txts{\textstyle}
\def\support{\mathrm{support}}
\def\varpic{\varpi^{\mathrm{c}}}
\def\final{n}

\def\target{\pi}
\def\statespace{\mathbb{X}}
% \def\xsp{\mathsf{X}}
\def\unit{\mathbf{1}}
\def\zero{\mathbf{0}}
\def\identity{\mathbf{I}}
\def\Utarget{\widetilde{\pi}}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\rmd{\mathrm{d}}
\def\tribu{\mathcal{B}(\mathcal{X})}
\def\param{\theta}
\def\paramspace{\Theta}
\def\transform{\mathrm{T}}
\def\indic{\mathbbm{1}}
\def\kernel{\mathrm{K}}
\def\pE{\mathbb{E}}
\def\pV{\mathbb{V}}
\def\transitionker{K_\target}
\def\gauss{\mathcal{N}}
% \def\Q{\mathrm{Q}}
\def\ula{\texttt{ULA}}
\def\mala{\texttt{MALA}}
\def\emalg{\texttt{EM}}
\def\rnvp{\texttt{RNVP}}
\def\P{\mu}
\def\heavy{h}
\def\1{\mathbbm{1}}
\def\probmeasures{\mathsf{M}_1}
\def\probmeasuresac{\mathsf{M}_{\target}}
\def\MCMCker{\mathrm{M}_\target}
\def\const{\mathcal{Z}}
\def\ratioQ{\mathcal{R}_\beta}
\def\bigo{\mathcal{O}}
\def\dkl{\mathbb{D}_{\mathrm{KL}}}
\def\distr{\mu}
\def\frakconst{\mathcal{Z}}
\def\student{\mathrm{Student}}
\def\paramfamily{\mathsf{F}_{\Theta}}
\def\kl{\mathrm{KL}}
\def\gm{\mathsf{GM}}
\def\rnvp{\mathtt{RNVP}}
\def\dontread{\textbf{\textcolor{red}{en chantier} }}
\def\localker{L_\target}
\def\pow{\varepsilon}
\def\half{\frac{1}{2}}
\def\EMC{\texttt{EM2C}}
\def\tbf{\textcolor{purple}{(To be finished.)}}
\def\projtarg{\target_*}
\def\renyiset{\mathsf{R}_{2,3}}
\def\infrenyiset{\mathsf{R}_\infty}
\def\Fmap{\mathcal{F}}
\def\Linf{\mathrm{L}^\infty}
\def\emFmap{\mathcal{F}_{\mathsf{em}}}
\def\eFmap{\mathcal{F}_{\mathsf{e}}}
\def\ulaker{\mathsf{R} _\gamma}
\def\lsconst{C_{\mathrm{LS}}}

\newcommand{\supnorm}[1]{\| #1 \|_\infty}
\newcommand{\skrenyi}[2]{\widetilde{\mathcal{R}}_{\target}(#1 \parallel #2)}
\newcommand{\ulaiterate}[1]{\iterate{#1}^{\mathsf{R}}}
\newcommand{\Fmc}[1]{\zeta^N _{#1}}
\newcommand{\constmu}[1]{\mathcal{Z}_{\iterate{#1}}}
\newcommand{\constmuK}[1]{\mathcal{Z}_{\iterate{#1} \transitionker}}
\newcommand{\mciterate}[1]{\mu^n _{#1}}
\newcommand{\gradinterpo}[1]{\overline{\nabla U}_{#1}}
\newcommand{\esssup}[1]{\mathrm{ess}\sup_{\lambda}}
\newcommand{\approxit}[1]{\mu_{\param _{#1}}}
\newcommand{\propo}[1]{\vartheta_{#1}}
\newcommand{\rnikodd}[3]{\frac{#1(#3)}{#2(#3)}}
% \newcommand{\rnikod}[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand{\proposalmap}{\vartheta}
\newcommand{\iterate}[1]{\mu_{#1}}
\newcommand{\iter}[3]{\Psi_{#1, #3}(#2)}
\newcommand{\tditerate}[1]{\tilde{\mu}_{#1}}
\newcommand{\sqmapping}[2]{
        \ifthenelse{\equal{#1}{}}
        {
            \mathcal{R}^{\pow,2} _{ #2}
            }
        {
            \mathcal{R}^{\pow_{#1}, 2} _ #2
            }}
\newcommand{\mapping}[2]{
        \ifthenelse{\equal{#1}{}}
        {
            \Psi^{\pow} _{ #2}
            }
        {
            \Psi^{\pow_{#1}} _{#2}
            }}
\newcommandx{\denoiser}[2][2=\param]{D^{#2} _{#1}}
\newcommandx{\score}[2][2=\param]{s^{#2} _{#1}}
\newcommandx{\scores}[2][2=\param]{s^{#2^{\star}} _{#1}}
\newcommand{\mixture}[1]{\mathcal{M}^\pow _{#1}}
% \newcommand{\uweight}[2]{\omega^{#1} _{#2}}
% \newcommand{\tv}[1]{\left\|#1\right\|_{\mathsf{TV}}}
\newcommand{\hatC}[1]{\widehat{\mathcal{C}}_{\target,#1}}
\newcommand{\urbetaK}[1]{\widetilde{\mathcal{R}}_{\beta, #1}}
\newcommand{\rbetaK}[1]{\mathcal{R}_{\beta, #1}}
\newcommand{\rbetaKstr}[1]{\mathfrak{R}_{\beta, #1}}
\newcommand{\ratio}[2]{\mathcal{R}_{#1}[#2]}
\newcommand{\ptheta}[1]{\mathrm{P}_{\param{#1}}}
% \newcommand{\particle}[2]{\xi^{#1} _{#2}}
\newcommand{\Tparticle}[2]{\widetilde{\xi}^{#1} _{#2}}
\newcommand{\paramiterate}[1]{\bar\mu_{\param#1}}
% \newcommand{\eqdef}{\ensuremath{:=}}
% \newcommand{\eqsp}{}
\newcommand{\piterate}[2]{\ifthenelse{\equal{#2}{}}{\hat\mu_{\param, #1}}{\hat\mu_{\param#2, #1}}}
% \newcommand{\weight}[1]{\omega_{#1}}
% \newcommand{\normweight}[2]{\mathcal{W}^{#1} _{#2}}
\newcommand{\borelians}[1]{\mathcal{B}(\mathbb{R}^{#1})}
\newcommand{\targetrestr}[1]{\target_{| #1}}
% \newcommand{\divergence}[3]{\mathcal{R}_{#1}(#2 \parallel #3)}
% \newcommand{\kldivergence}[2]{\mathsf{KL}(#1 \parallel #2)}
\newcommand{\pushptheta}[2]{#1_{\#} \ptheta{#2}}
\newcommand{\C}[1]{\mathcal{C}_{\target, #1}}
\newcommand{\sumC}[1]{\mathcal{S} _{#1}}
\newcommand{\UsumC}[1]{\widetilde{\mathcal{S}} _{#1}}
\newcommand{\hatsumC}[2]{\widehat{\mathcal{S}}^{#2} _{#1}}
\newcommand{\hatUsumC}[2]{\widehat{\mathsf{S}}^{\mathrm{u} #2} _{#1}}
\newcommand{\A}[2]{\ifthenelse{\equal{#2}{}}{(\textbf{A}{\textbf{\ref{#1})}}}{(\textbf{A}\textbf{\ref{#1}-\ref{#2}})}}
\newcommand{\assp}[1]{(\textbf{A}\textbf{#1})}
\newcommand{\average}[1]{\mathcal{A}_{\beta, #1}}
\newcommand{\law}[1]{\mathsf{Law}(#1)}

%mcgdiff notations

\def\obs{y}
\newcommand{\iobs}[1]{{\obs_\tstep{#1}}}
\def\nsteps{S}
\def\cov{\mathbb{C}\mathrm{ov}}
\def\covobs{\Sigma_\obs}
\def\obsrv{Y}
\def\rmd{\mathrm{d}}
\def\pP{\mathbb{P}}
\def\noise{\varepsilon}
\def\noiserv{Z}
\def\pE{\mathbb{E}}
\def\pV{\mathbb{V}}
\def\ltrstate{x}
% \def\eqdef{:=}
\def\baseset{\Omega}
\def\basesigma{\mathcal{F}}
\def\baseprob{\mathbb{P}}
\def\eqsp{\,}
\def\1{\mathbbm{1}}
\def\dimx{{d_{x}}}
\def\dimz{d_z}
\def\dimy{d_y}
% \def\dimtr{{\smash{\overline{d}}}}
\def\dimtr{\mathsf{t}}
\newcommand{\numsqrt}[1]{\smash{#1}^{1/2}}
\def\dimorig{{d_{\mathbf{y}}}}
% \def\dimb{\smash{\underline{d}}}
\def\dimb{\mathsf{b}}
\def\trmeas{Y}
\def\ltrmeas{y}
\def\ormeas{\mathbf{Y}}
\def\lmeas{\mathbf{y}}
\def\revmeas{\overleftarrow{Y}}
\def\state{\mathbf{X}}
\def\diffltrmeas{\mathsf{\ltrmeas}}
\def\trstate{X}
\def\rset{\mathbb{R}}
\def\nset{\mathbb{N}}
\def\nsetpos{\mathbb{N}_*}
\def\idm{\operatorname{I}}
\def\nlessc{\m{J}^0}
\def\top{\mathsf{t}}
\def\bot{\mathsf{b}}
\def\nyc{\m{J}}
\newcommand{\m}[1]{\operatorname{#1}}
\newcommand{\cat}[2]{{#1}^{\scriptscriptstyle\frown}#2}
\newcommand{\vect}[1]{\mathbf{#1}}
% \DeclareMathOperator*{\argmin}{argmin}
\def\gauss{\mathcal{N}}
\def\noise{\varepsilon}
\def\R{\mathbb{R}}
\def\bV{\mathbf{V}}
% \DeclareMathOperator*{\argmax}{argmax}
\def\bY{\mathbf{Y}}
\def\stateperp{\mathbf{x}^\perp}
\def\stateperp{\bm{\xi}^\perp}
\def\invX{\xi}
\def\perpstate{\bm{\xi}}
\def\parallelstate{\bm{\zeta}}
% \def\datadistr{\pi_*}
\def\param{\theta}
\def\sigalgebra{\mathcal{B}}
\def\normpdf{\mathcal{N}}
% \def\normpdf{\phi}
\def\normdist{\mathcal{N}}
\def\normconst{\mathcal{Z}}
\def\sumweights{\Omega}
\def\boundedfunc{\mathsf{F}}
\def\bigo{\mathcal{O}}
\def\eigSigmay{\sigma^y}
\def\eigA{\sigma^A}
\def\id{\mathbf{I}}
\def\categorical{\mathrm{Categorical}}
\def\ouralgorithm{\algo}
\def\motif{\mathcal{M}}
\def\scaffold{\mathcal{S}}
% \newcommand{\card}[1]{|#1|}
\newcommand{\floor}[1]{{\lfloor #1 \rfloor}}
\newcommand{\eigsigy}[1]{\sigma_{y, #1}}
\newcommand{\twodvect}[2]{(#1, #2)}
\newcommand{\xblock}[2]{x^{B_{#2}} _{#1}}
\newcommand{\filtration}[1]{\mathcal{F}_{#1}}
\newcommand{\fwdker}[3]{\overrightarrow{\mathbf{B}}_{#1}(#2 #3)}
% \newcommand{\uweight}[2]{\widetilde{\omega}^{#1} _{#2}}
% \newcommand{\weight}[2]{\omega^{#1} _{#2}}
\newcommand{\wratio}[3]{\frac{\tilde{\omega}^{#1} _{#2}(#3)}{\Omega^N _{#2}}}
% \newcommand{\kldivergence}[2]{\mathsf{KL}(#1 \parallel #2)}
\def\prtcl{\xi}
\def\tparticle{\smash{\overline{\prtcl}}}
\def\bparticle{\smash{\underline{\prtcl}}}
\newcommand{\iparticle}[2]{x^{#1} _{#2}}
\newcommand{\mset}[2]{\R^{#1 \times #2}}
\newcommand{\X}[1]{X_{#1}}
% \newcommand{\statevar}[1]{\ifthenelse{\equal{#1}{}}{\mathbf{x}}{\mathbf{x}_{#1}}}
\newcommand{\statevar}[1]{\mathbf{x}_{#1}}
% \newcommand{\statevar}[1]{\ifthenelse{\equal{#1}{1}}{\mathbf{x}}{\mathbf{x}_{#1}}}
% \newcommand{\statevar}[1]{\mathbf{x}_{#1}}
\newcommand{\Y}[1]{Y_{#1}}
\newcommand{\revX}[1]{\overset{{}_{\leftarrow}}{X} _{#1}}
\newcommand{\revY}[1]{Y_{#1}}
\newcommand{\W}[1]{W_{#1}}
\newcommand{\condprob}[2]{\baseprob\left(#1|#2\right)}
% \newcommand{\scorenet}[3]{\mathbf{s}_{#1}(#2, #3)}
\newcommand{\zerom}[2]{\mathbf{0}_{#1, #2}}
\def\noisestd{\sigma}
\def\tbw{...}
\def\orthdatadistr{\tilde{\pi}_{*}}
\newcommandx{\acp}[2][2=]{\ifthenelse{\equal{#2}{}}{\alpha_{#1}}{\alpha_{#1:#2}}}
\newcommand{\fwsigma}[2]{\sigma_{#1,#2}}
%  \newcommand{\eric}[1]{\todo[color=blue!20]{{\bf E:} #1}}
 \newcommand{\erici}[1]{\todo[inline,color=blue!20]{{\bf E:} #1}}
% \newcommand\gabriel[1]{\todo[color=green!20]{{\bf G:} #1}}
% \newcommand\yazid[1]{\todo[color=red!20]{{\bf Y:} #1}}
\newcommand\syl[1]{\todo[color=red!60]{{\bf Syl:} #1}}
\newcommandx{\xpred}[2][2=]{\boldsymbol{\chi}^{#2} _{#1}}
\newcommandx{\bottomxpred}[2][2=]{\underline{\boldsymbol{\chi}}^{#2} _{#1}}
\newcommandx{\topxpred}[2][2=]{\overline{\boldsymbol{\chi}}^{#2} _{#1}}
\newcommand{\ndist}[2]{\mathcal{N}(#1, #2)}
\newcommand{\soset}[1]{\operatorname{SO}(#1)}
\newcommand{\tstatevar}[1]{\overline{\mathbf{x}} _{#1}}
\newcommand{\bstatevar}[1]{\underline{\mathbf{x}} _{#1}}
\newcommand{\tstate}[1]{\overline{\state} _{#1}}
\newcommand{\bstate}[1]{\underline{\state} _{#1}}
\newcommand{\tcr}[1]{\textcolor{red}{#1}}
% \newcommand{\prior}[1]{p_{#1}}
% \newcommand{\proposal}[2]{p_{#1, #2}}
\newcommand{\predstartprop}[2]{f_{#2}(#1)}
\newcommand{\epsprop}[2]{\ifthenelse{\equal{#1}{}}{\mathbf{e}^{#2}}{\mathbf{e}^{#2} (#1)}}
\newcommand{\vecidx}[3]{#1 _{#2}[#3]}
\newcommand{\expec}[2]{\mathbb{E}_{ #1}\left[#2\right]}
\newcommand{\realrevbridge}[3]{\ifthenelse{\equal{#2}{}}{\mathsf{q} _{#1}}{\mathsf{q} _{#1}(#3|#2)}}
\newcommand{\revbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{{q}}^{\sigma} _{#1}}{\smash{{q}}^{\sigma} _{#1}(#3|#2)}}
\newcommand{\idxrevbridge}[4]{\ifthenelse{\equal{#2}{}}{\smash{{q}}^{\sigma, #4} _{#1}}{\smash{{q}}^{\sigma, #4} _{#1}(#3|#2)}}
\newcommand{\trevbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{\overline{q}}^{\sigma} _{#1}}{\smash{\overline{q}}^{\sigma} _{#1}(#3|#2)}}
\newcommand{\brevbridge}[3]{\ifthenelse{\equal{#2}{}}{\underline{q}^{\sigma} _{#1}}{\underline{q}^{\sigma} _{#1}(#3|#2)}}
% \newcommand{\realrevbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{\overset{{}_{\leftarrow}}{q}^{\sigma_*}} _{#1}}{\smash{\overset{{}_{\leftarrow}}{q}}^{\sigma_*} _{#1}(#3|#2)}}
% \newcommand{\proposal}[2]{\overleftarrow{q}_{#1,#2}}
\newcommand{\bwproposal}[1]{\overleftarrow{Q}^{#1}}
\newcommand{\ouproposal}[1]{\overrightarrow{P}^{#1}}
\newcommand{\bridge}[4]{{\ifthenelse{\equal{#3}{}}{p^{#2} _{#1}}{p^{#2} _{#1}(#3, #4)}}}
\newcommand{\outrans}[3]{\ifthenelse{\equal{#2}{}}{\overrightarrow{m}_{#1}}{\overrightarrow{m}_{#1}(#2, #3)}}
% \newcommand{\bw }[4]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{m}^{#1}} _{#2}}{\smash{\overset{{}_{\leftarrow}}{m}}^{#1} _{#2}(#4|#3)}}
\newcommandx{\bw }[4][4=]{\ifthenelse{\equal{#3}{}}{q^{#4} _{#1}}{q^{#4} _{#1}(#3|#2)}}
\newcommandx{\fw}[4][4=]{\ifthenelse{\equal{#3}{}}{q^{#4} _{#1}}{q^{#4} _{#1}(#3|#2)}}
\newcommandx{\rbwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{q}^{#4} _{#1}}{\smash{q}^{#4} _{#1}(#3|#2)}}
\newcommandx{\pbwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\hat{p}^{#4} _{#1}}{\hat{p}^{#4} _{#1}(#3|#2)}}
\newcommandx{\abwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{p}^{#4} _{#1}}{\smash{p}^{#4} _{#1}(#3|#2)}}
\newcommandx{\pibw}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\target}^{#4} _{#1}}{\smash{\target}^{#4} _{#1}(#3|#2)}}
\newcommandx{\hbwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\hat{q}}^{#4} _{#1}}{\smash{\hat{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\cabwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{q}^{#4} _{#1}}{\smash{q}^{#4} _{#1}(#3|#2)}}
\newcommandx{\aabwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\tilde{q}}^{#4} _{#1}}{\smash{\tilde{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\vbwker}[4][4=\vparam]{\ifthenelse{\equal{#3}{}}{\pi^{#4} _{#1}}{\pi^{#4} _{#1}(#3|#2)}}
\newcommandx{\hpibw}[4][4=\ell]{\ifthenelse{\equal{#3}{}}{\smash{\hat\pi^{#4} _{#1}}}{\smash{\hat\pi^{#4} _{#1}(#3|#2)}}}
\newcommandx{\hmrg}[2][2=\ell]{\smash{\hat\pi^{#2} _{#1}}}
\newcommandx{\cbwtrans}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\Pbwtrans}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{P}}^{#4} _{#1}}{\smash{\overset{{}_{\leftarrow}}{P}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\condbw}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\fwtrans}[4][4=]{\ifthenelse{\equal{#2}{}}{q_{#1}}{q _{#1}(#3|#2)}}
\newcommandx{\cbwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{q^{#3} _{#1}}{q^{#3}_{#1}(#2)}}
\newcommandx{\bwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{p^{#3} _{#1}}{p^{#3}_{#1}(#2)}}
\newcommand{\bwoptmarg}[3]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{{\mathfrak{m}}}}^{#2} _{#1}}{\smash{\overset{{}_{\leftarrow}}{{\mathfrak{m}}}}^{#2} _{#1}(#3)}}
\newcommandx{\fwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{q^{#3} _{#1}}{q^{#3} _{#1}(#2)}}
\newcommandx{\cfwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{q^{#3} _{#1}}{q^{#3} _{#1}(#2)}}
\newcommand{\posterior}[2]{\ifthenelse{\equal{#2}{}}{p^\obs _{#1}}{p^\obs _{#1}(#2)}}
\newcommand{\initdistr}[3]{\ifthenelse{\equal{#2}{}}{\chi_{#1}}{\chi_{#1}(#2, #3)}}
% \newcommand{\bwopt}[4]{{\ifthenelse{\equal{#3}{}}{\overleftarrow{m}^{#2} _{#1}}{\overleftarrow{m}^{#2} _{#1}(#3 #4)}}}
\newcommand{\bwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{p^{#2} _{#1}(#4|#3)}}
\newcommand{\bbwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{\underline{p}^{#2} _{#1}(#4|#3)}}
\newcommand{\tbwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{\overline{p}^{#2} _{#1}(#4|#3)}}
\newcommand{\fwopt}[4]{\ifthenelse{\equal{#3}{}}{\overset{{}_{\rightarrow}}{m} ^{#2} _{#1}}{\smash{\overset{{}_{\rightarrow}}{m}}^{#2} _{#1}(#4|#3)}}
\newcommand{\ufilter}[3]{{\ifthenelse{\equal{#3}{}}{\eta^{#2} _{#1}}{\eta^{#2} _{#1}(#3)}}}
\newcommand{\filter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi^{#2} _{#1}(#3)}}}
\newcommand{\noisyfilter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi^{#2} _{#1}(#3)}}}
\newcommand{\noiselessfilter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi _{#1}(#3 | #2)}}}
% \newcommand{\pred}[3]{{\ifthenelse{\equal{#3}{}}{\eta^{#2} _{#1}}{\eta^{#2} _{#1}(#3)}}}
\newcommand{\bfilter}[3]{{\ifthenelse{\equal{#3}{}}{\Phi^{#2} _{#1}}{\Phi^{#2} _{#1}(#3)}}}
\newcommand{\normconstest}[1]{\gamma^N _{#1}}
\newcommand{\Qker}[2]{Q_{#1} ^{#2}}
\newcommand{\lawSMC}[1]{P^N _{#1}}
\newcommand{\lawcSMC}[1]{\mathbf{P}^N _{#1}}

% \newcommand{\anc}[2]{\smash{A^{#1} _{#2}}}
\newcommand{\ianc}[2]{a^{#1} _{#2}}
\newcommand{\iancanc}[2]{b^{#1} _{#2}}
\newcommand{\pot}[3]{\ifthenelse{\equal{#3}{}}{\smash{g^{#2} _{#1}}}{\smash{g^{#2} _{#1}}(#3)}}
\newcommand{\ipot}[3]{\ifthenelse{\equal{#3}{}}{g^{#2} _{#1}}{g^{#2} _{#1}(#3)}}
\newcommand{\iapot}[3]{\ifthenelse{\equal{#3}{}}{\tilde{g}^{#2} _{#1}}{\tilde{g}^{#2} _{#1}(#3)}}
\newcommand{\dubpot}[3]{\ifthenelse{\equal{#3}{}}{G^{#2} _{#1}}{G^{#2} _{#1}(#3)}}
\newcommand{\fwfilter}[1]{\eta^{\ltrmeas} _{#1}}
% \newcommand{\dforward}[1]{\overrightarrow{m}_{#1}}
% \newcommand{\dbackward}[1]{\overleftarrow{m}_{#1}}
% \newcommand{\pot}[1]{g_{#1}}
% \newcommand{\optforward}[1]{\overrightarrow{p _{#1}}}
% \newcommand{\optbackward}[1]{\overleftarrow{p _{#1}}}
\newcommand{\couplepot}[1]{\mathrm{G}_{#1}}
\newcommand{\intvect}[2]{[#1:#2]}
\def\pathmforward{\overrightarrow{\lambda}}
\def\pathmbackward{\overleftarrow{\lambda}}
% \newcommand{\assp}[1]{(\textbf{A}\textbf{#1})}
\newcommand{\clipleb}[3]{\nu^{#2} _{#1}(#3)}
\newcommand{\noisytrans}[3]{\ifthenelse{\equal{#2}{}}{\mathsf{P}_{#1}}{\mathsf{P}_{#1}(#3|#2)}}
% \def\algo{\texttt{MCGdiff}}
\def\ddrm{DDRM}
\def\dps{\texttt{DPS}}
\def\smcdiff{\texttt{SMCdiff}}
\def\ddim{\texttt{DDIM}}
\def\dimg{d}
%\newcommand{\chunk}[3]{{#1}_{#2}^{#3}}
\newcommand{\pchunk}[3]{#1 ^{#2:#3}}
\newcommand{\philter}[2]{\phi_{#1} ^{#2}}
\def\Id{\mathbf{I}}
%\def\Id{I}
\def\ltopstate{\overline{x}}
\def\lbotstate{\underline{x}}
\def\topstate{\smash{\overline{X}}}
\def\bottomstate{\underline{X}}
% \newcommandx\sequence[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2} \}_{#2 \in #3}}}}
\newcommand\projidx[3]{\ifthenelse{\equal{#2}{}}{#1^{\setminus #3}}{#1^{\setminus #3}_{#2}}}
\newcommand\insertidx[3]{#1^{#2, #3}}

\newcommand{\fwpGen}[1]{p^\genparam _{#1}}
\newcommand{\tstep}[1]{{k_{#1}}}
\newcommand{\ustate}[2]{X^{#1} _{#2}}
\newcommand{\lstate}[2]{X^{#1} _{#2}}
\newcommand{\post}[2]{\ifthenelse{\equal{#2}{}}{\pi_{#1}}{\pi_{#1}(#2)}}
\newcommand{\potn}[2]{\ifthenelse{\equal{#2}{}}{g_{#1}}{g_{#1}(#2)}}
\newcommand{\hpotn}[2]{\ifthenelse{\equal{#2}{}}{\hat{g}_{#1}}{\hat{g}_{#1}(#2)}}
\def\tmidfn{\ell}
\newcommand{\tmid}[1]{{\tmidfn_k}}
\newcommandx{\vmu}[1][1=]{\hat\mu^{#1}}
\newcommandx{\vstd}[1][1=]{\hat\sigma^{#1}}
\newcommandx{\vlstd}[1][1=]{\hat\upsilon^{#1}}
\def\vparam{\varphi}
\def\stdq{\sigma_q}
\def\muq{\mu_q}
\newcommand{\std}[1]{\sigma_{#1}}
\newcommand{\var}[1]{\sigma^2 _{#1}}
\newcommand{\mean}[1]{m_{#1}}
\def\vvparam{\psi}
\def\optparam{\param_\star}
%\def\diag{\mathrm{diag}}
\def\diag{\mbox{diag}}

\newcommand{\vub}[1]{\mathcal{L}_{#1}}

%%%%%%%%%%%%%%%%%%%%%
%% mathbf
%\def\bfA{\mathbf{A}}
\def\bfA{A}
\def\bfC{\mathbf{C}}

\newcommand{\tcr}[1]{\textcolor{red}{#1}}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/background.tex <==
We provide a brief overview of DDMs \cite{sohl2015deep,song2019generative,ho2020denoising}. Suppose we can access an empirical sample from some data distribution $\datadistr$ defined on $\rset^{\dimx}$. %Rather than directly approximating this distribution, DDMs learn to denoise the data distribution corrupted with increased levels of noise. The learned denoisers are then leveraged to construct a Markov chain that samples approximately from $\datadistr$.
For every $k \in \nset$, define the distribution $\fwmarg{k}{\bx _k} \eqdef \int \datadistr(\bx _0) \, \fwtrans{k|0}{\bx _0}{\bx _k} \rmd \bx _0$ with $\fwtrans{k|0}{\bx _0}{\bx _k} \eqdef \normpdf(\bx _k; \sqrt{\acp{k}} \bx _0, (1 - \acp{k})\Id_\dimx)$, where
%\begin{equation}
%    \label{eq:fwd_process}
%    \fwtrans{t|0}{\bx _0}{\bx _t} \eqdef \normpdf(\bx _t; \sqrt{\acp{t}} \bx _0, (1 - \acp{t} )\Id_\dimx)
%\end{equation}
$(\acp{k})_{k \in \nset}$ is a sequence that tends to zero as $t$ tends to infinity, with $\alpha_0 = 1$.
%(having the same dimension than the input $\bx$).
The probability density $\fwmarg{k}{}$ corresponds to the marginal distribution at time $k$ of an auto-regressive process on $\rset^{d_x}$ given by $\bX _{k + 1} = \sqrt{\acp{k+1} / \acp{k}} \bX _k + \sqrt{1 - \acp{k + 1} / \acp{k}} \beps_{k + 1}$, $k \in \nset$, with $\bX _0 \sim \datadistr$ and $(\beps_k)_{k \in \Npos}$ being a sequence of {\iid} $\dimx$-dimensional standard normal random variables.
%$\gauss(\zero_{\dimx}, \Id_{\dimx})$.

DDMs leverage parametric approximations $\smash{\predx{k}[\param]}$ of the mappings $\smash{\bx _k \mapsto \int \bx _0 \, \bw {0|k}{\bx _k}{\bx _0} \rmd \bx _0}$, where $\bw {0|k}{\bx _k}{\bx _0} \propto \datadistr(\bx _0) \fwtrans{k|0}{\bx _0}{\bx _k}$ is the conditional distribution of $\bX _0$ given $\bX _k = \bx _k$. Each $\predx{k}[\param]$ is defined as $\predx{k}[\param](\bx _k) \eqdef (\bx _k - \sqrt{1 - \acp{k}} \prednoise{k}(\bx _k)) / \sqrt{\acp{k}}$, where $\prednoise{k}$ is a noise predictor network trained by minimizing a denoising objective; see \cite[Eq.~(12)]{ho2020denoising} for details. Following \cite[Section 4.2]{dhariwal2021diffusion}, $\prednoise{k}$ also provides an estimate of the score $\nabla \log \fwmarg{k}{\bx _k}$ given by $\score{k}[\param](\bx _k) \eqdef -\big(\bx _k - \sqrt{\acp{k}}\predx{k}[\param](\bx _k)\big) / (1 - \acp{k})$.
We denote by $\param^\star$ the minimizer of the denoising objective.
Having access to $\param^\star$, we can define a generative model for $\datadistr$ by adopting the denoising diffusion probabilistic model (DDPM) framework of \cite{ho2020denoising}
We assume that $n$ is large enough so that $\fwmarg{n}{}$ is approximately multivariate standard normal.
Define the \emph{bridge kernel} $\fwtrans{k|0, k+1}{\bx _0, \bx _{k+1}}{\bx _k} \propto \fwtrans{k|0}{\bx _0}{\bx _k} \fwtrans{k+1|k}{\bx _k}{\bx _{k+1}}$ which is a Gaussian distribution with mean $\muDDIM{k|0, k+1}(\bx _0, \bx _{k+1})$ and diagonal covariance $\sigma^2 _{k|k+1} \Id_\dimx$ defined in \Cref{apdx:ddim}.
Then for every $k \in \intset{1}{n-1}$ we define the backward transition densities
\begin{equation}
    \label{eq:ddpm_kernel}
\abwker{k|k+1}{\bx _{k+1}}{\bx _k}[\theta^{\star}] \eqdef \fwtrans{k|0, k+1}{\predxs{k+1}(\bx _{k+1}), \bx _{k+1}}{\bx _k}\eqsp,
\end{equation}
% %\begin{equation}
% %    \label{eq:mean_ddim}
% %    \muDDIM{k|0, k+1}(\bx _0, \bx _{k+1}) \eqdef \acp{k}^{1/2} \bx _0 + (1 - \acp{k} - \sigma^{2} _{k|k+1})^{1/2} (1 - \acp{k+1})^{-1/2} (\bx _{k+1} - \acp{k+1} \bx _0)
% %\end{equation}
% \begin{equation}
%     \label{eq:mean_ddim}
%     \muDDIM{k|0, k+1}(\bx _0, \bx _{k+1}) \eqdef \sqrt{\acp{k}} \bx _0 + \sqrt{(1 - \acp{k} - \sigma^{2} _{k|k+1}) / (1 - \acp{k+1})} (\bx _{k+1} - \acp{k+1} \bx _0)
% \end{equation}
% and  $\sigma^2_{k|k+1} \eqdef \eta^2 (1 - \acp{k}) (1 - \acp{k+1} / \acp{k}) \big/ (1 - \acp{k+1})$;
% see \citet{song2021denoising}.
and $\abwker{0|1}{\bx _1}{\cdot}[\theta^{\star}] \eqdef \delta_{\predxs{1}(\bx _1)}$. On the basis of these transition densities, we define the joint distribution
\begin{equation}
    \label{eq:ddim_joint}
    \txts \bwmarg{0:n}{\bx _{0:n}}[\theta^{\star}] = \bwmarg{n}{\bx _n} \prod_{k = 0}^{n-1} \abwker{k|k+1}{\bx _{k+1}}{\bx _k}[\theta^{\star}] \eqsp,
\end{equation}
where $\bwmarg{n}{\bx _n} = \normpdf(\bx _n ; 0,\Id_{\dimx})$.
%$\bwmarg{n}{}= \gauss(0,\Id_{\dimx})$.
%We let $\muDDIM{k|k+1}(\bx _{k+1})= \muDDIM{k|0,k+1}(\predxs{k+1}(\bx _{k+1}),\bx _{k+1}) $; see \eqref{eq:mean_ddim}.\jimmy{I cannot see that this notation is used in the paper? (At least not in the main corpus.)}
In the following we assume that we have access to a trained DDM, and expunge the superscript $\theta^{\star}$ from the notation, writing simply $\bwmarg{}{}$ and $\smash{\predx{k}[]}$ when referring to the generative model and the denoiser, respectively. In addition, we denote by $\smash{\bwmarg{k}{}[]}$ the $k$-th marginal of $\bwmarg{0:n}{}[]$ and write, for all $(\ell, m) \in \intset{0}{n}^2$ such that $\ell < m$, $\abwker{\ell|m}{\bx _m}{\bx _\ell} \eqdef \prod_{k = \ell} ^{m-1} \abwker{k|k+1}{\bx _{k+1}}{\bx _k}$.

==> sections/def.tex <==
\def\algo{\sc{VDPS}}
\def\algoname{{\sc{Variational Diffusion Posterior sampler}}}
\def\tauks{L}
\def\PGDM{\Pi \mathrm{GDM}}
\def\DPS{DPS}
\def\imsize{=0.2\hsize}
% \def\eqdef{\ensuremath{:=}}
\def\eqdef{\vcentcolon=}
\def\IP{\mathrm{IP}}
\def\mcgdiff{MCGDiff}
\def\target{\pi}
\def\prior{q}
\def\normconst{\mathcal{Z}}
\def\Idmat{\mathbf{I}}
\def\KL{\mathsf{KL}}
\def\data{Y}
\def\Yspace{\mathsf{Y}}
\def\datadistr{q}
\def\rset{\mathbb{R}}
\def\nset{\mathbb{N}}
\def\rmd{\mathrm{d}}
\def\latent{X}
\def\approxdistr{\operatorname{Q}}
\def\datvar{y}
\def\latvar{x}
\def\eqsp{}
%\def\eqsp{\,}
\def\pV{\mathbb{V}}
\def\pE{\mathbb{E}}
\def\gauss{\mathcal{N}}
\def\N{\mathbb{N}}
\def\Npos{\mathbb{N}_{>0}}
\def\param{\theta}
\def\paramspace{\Theta}
\def\probmeasures{\mathbb{M}_1}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\def\dimobs{{d_\obs}}
\def\dimlatent{p}
\def\Ysigalgebra{\mathcal{Y}}
\def\Xspace{\mathsf{X}}
\def\Xsigalgebra{\mathcal{X}}
\def\variationalfamily{\mathcal{F}}
\def\targetdistr{\pi}
\def\transform{\operatorname{T}}
\def\phispace{\mathsf{T}}
\def\categorical{\mathrm{Categorical}}
\def\1{\mathbbm{1}}
\def\FFBS{\mathrm{FFBS}}
\def\FFBSi{\mathrm{FFBSi}}
\def\PARIS{\mathrm{PaRIS}}
\def\BS{\mathsf{BS}}
\def\bigo{\mathcal{O}}
\newcommandx{\generator}[1][1=]{G^{\genparam _{#1}}}
\def\genparam{\varphi}
\def\pGen{p_\genparam}
\newcommandx{\bwreparam}[1][1=]{\mathcal{G}^{\genparam_{#1}}}
\def\Xset{\mathsf{X}}
\def\Yset{\mathsf{Y}}
\def\sigmaX{\mathcal{X}}
\def\sigmaY{\mathcal{Y}}
\def\1{\mathbbm{1}}
\def\T{\mathrm{\mathbf{T}}}
\def\G{\mathrm{\mathbf{G}}}
\def\pE{\mathbb{E}}
\def\pP{\mathbb{P}}
\def\pV{\mathbb{V}}
\def\N{\mathbb{N}}
\def\plim{\overset{\pP}{\longrightarrow}}
\def\dlim{\Longrightarrow}
\def\gauss{\mathcal{N}}
% \def\cat{\textrm{Cat}}
\def\XX{\mathrm{XX}}
\def\GT{\mathsf{GT}}
\def\BS{\mathsf{BS}}
\def\rmd{\mathrm{d}}
\def\R{\mathbb{R}}
\def\rhs{r.h.s.}
\def\aslim{\overset{a.s.}{\underset{N \to \infty}{\longrightarrow}}}
\def\backsum{\mathcal{T}}
\def\sett{\mathcal{S}}
\def\eve{\mathrm{E}}
\def\Bset{\mathcal{B}}
\def\zero{\mathbf{0}}
\def\bigo{\mathcal{O}}
\def\boldone{\mathbf{1}}
% \def\FFBS{\mathrm{FFBS}}
% \def\FFBSi{\mathrm{FFBSi}}
\def\weightmat{\overline{\mathcal{W}}}
\def\roundW{\mathcal{W}}
\def\simplelim{\underset{N \to \infty}{\lim}}
\def\boundg{G_\infty}
\def\paris{\textit{PaRIS}}
\def\Pbacksum{\widetilde{\backsum}}
\def\bigH{\textbf{H}}
\def\bigF{\textbf{F}}
\def\pos{\mathsf{Pos}}
\def\stdobs{\sigma_\obs}
\def\ft{T}
\def\last{n}
\def\lasto{K}
\def\gvf{\mathcal{G}}
\def\dgvf{\mathcal{G}_\mathrm{D}}
\def\eqinlaw{\smash{\overset{\mathcal{L}}{=}}}
% \def\vmu{\mu^\vparam}
% \def\vstd{\sigma^\vparam}

\newcommand{\stdiobs}[1]{\sigma _{\obs, {#1}}}
\newcommand{\intset}[2]{\llbracket #1, #2 \rrbracket}
\newcommand{\lklhd}[2]{\ifthenelse{\equal{#2}{}}{g^\obs _{#1}}{g^\obs _{#1}(#2)}}
\newcommand{\change}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{\small{#1}}}
\newcommand{\todoo}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{\small{#1}}}
\newcommand{\sylvain}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{\small{\textbf{S} :#1}}}
\newcommand{\jimmy}[1]{\todo[linecolor=magenta,backgroundcolor=magenta!25,bordercolor=magenta]{\tiny{\textbf{JO} : \ #1}}}
\newcommand{\yazid}[1]{\textcolor{blue}{\textbf{YJ}: #1}}
\newcommand{\alain}[1]{\todo[linecolor=cyan,backgroundcolor=cyan!25,bordercolor=cyan]{\small{\textbf{A} :#1}}}
\newcommand{\yohan}[1]{\todo[linecolor=purple,backgroundcolor=purple!25,bordercolor=purple]{\small{\textbf{YP}: #1}}}
\newcommand{\julien}[1]{\todo[linecolor=purple,backgroundcolor=purple!25,bordercolor=purple]{\small{\textbf{J}: #1}}}


\newcommand{\anc}[2]{\smash{A^{#1} _{#2}}}
\newcommand{\yazidd}[1]{\todo[color=blue!20]{{\bf Y:} #1}}
\newcommand{\badr}[1]{\todo[color=red!20]{{\bf B:} #1}}
\newcommand{\divergence}[3]{\mathcal{R}_{#1}(#2 \parallel #3)}
\newcommand{\uweight}[2]{\indx{\widetilde{\omega}}{#1}{#2}}
\newcommand{\weight}[2]{\indx{\omega}{#1}{#2}}
\newcommand{\rnikod}[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand{\flatrnikod}[2]{\rmd #1 / \rmd #2}
\newcommand{\tmidest}[1]{\smash{\target^M _{#1}}}
\newcommand{\SNISest}[1]{\smash{\overline{\target}^M _{#1}}}
\newcommand{\SIRest}[1]{\smash{\widetilde{\target}^M _{#1}}}
\newcommand{\tmiddistr}[4]{\nu^{#1} _{#2}(#4|#3)}
\newcommand{\kldivergence}[2]{\mathsf{KL}(#1 \parallel #2)}
\newcommand{\indx}[3]{#1^{#2} _{#3}}
% \newcommand{\chunk}[3]{#1^{#2:#3}}
\newcommand{\flatchunk}[3]{(\idx{#1}{#2}{}, \dotsc, \idx{#1}{#3}{})}
\newcommand{\Qdistr}[4]{\ifthenelse{\equal{#4}{}}{q^{#1} _{#2}}{q^{#1} _{#2}(#4 |#3)}}
\newcommand{\mudistr}[4]{\ifthenelse{\equal{#4}{}}{\mu^{#1} _{#2}}{\mu^{#1} _{#2}(#4 |#3)}}
\newcommand{\Qpost}[3]{\ifthenelse{\equal{#3}{}}{q^{#1} _{\latent|\data}}{q^{#1} _{\latent|\data}(#3 |#2)}}

\newcommand{\reviewed}[1]{\textcolor{blue}{#1}}
\newcommand{\Const}[1]{\mathcal{C}_{N,b,#1}}
\newcommand{\Gfilt}[2]{\mathcal{G}^N _{#2}}
\newcommand{\proj}[2]{\mathrm{\Pi}_{#1,#2}}
\newcommand{\Gsigma}[2]{\mathcal{G}^{#2}_{#1}}
\newcommand{\card}[1]{\mathrm{Card}(#1)}
\newcommand{\bigprod}[1]{\overline{\Lambda}^{1,2} _{#1}}
\newcommand{\intersect}[2]{\mathrm{I}_{#1}(#2)}
\newcommand{\joint}[1]{\gamma _{#1}}
\newcommand{\pred}[1]{\eta _{#1}}
\newcommandx{\predx}[3][2=0,3=\param]{\hat{x}^{#3} _{#2|#1}}
\newcommandx{\bwmean}[1]{m_{#1}}
\newcommandx{\bwvar}[1]{\sigma_{#1}}
\newcommandx{\predxs}[3][2=0,3=\optparam]{\hat{x}^{#3} _{#2|#1}}
\newcommandx{\prednoise}[2][2=\param]{\smash{\hat{\epsilon}^{#2} _{#1}}}
% \newcommand{\filter}[1]{\phi _{#1}}
\newcommand{\F}[1]{\mathcal{F}^N _{#1}}
\newcommand{\GG}[1]{\mathrm{\mathbf{G}}_{#1}}
\def\forward{\mathrm{f}}
\def\backward{\mathrm{b}}
\def\L{\mathrm{\mathbf{L}}}
\newcommand{\smooth}[2]{\phi_{#1 | #2}}
\newcommand{\smoothN}[3]{\phi^{#3} _{#1 | #2}}
\newcommand{\particletraj}[2]{\xi^{#1 _{0:#2}} _{0:#2}}
\newcommand{\particlecloud}[1]{\bm \xi^{1:N} _{0:#1}}
\newcommand{\bwker}[1]{\mathrm{\mathbf{B}} _{\phi_{#1}}}
\newcommand{\bwpath}[1]{\mathrm{\mathbf{T}} _{#1}}
\newcommand{\transition}[1]{\ifthenelse{\equal{#1}{0}}{M_0}{M_{#1}}}
\newcommand{\fakeprior}{\gamma}
\newcommand{\Q}[1]{\mathrm{\mathbf{Q}}_{#1}}
\newcommand{\Qmarg}[1]{\overline{\mathrm{\mathbf{Q}}}_{#1}}
\newcommand{\asymptvarest}[2]{\ifthenelse{\equal{#2}{}}{\ensuremath{\Gamma _{0: #1 \mid #1}}}{\ensuremath{\Gamma^{#2}_{0: #1 \mid #1}}}}
\newcommand{\asymptvarffbs}[2]{\ifthenelse{\equal{#2}{}}{\ensuremath{\Gamma^{\textrm{FFBS}} _{0: #1 \mid #1}}}{\ensuremath{\Gamma^{#2, \textrm{FFBS}}_{0: #1 \mid #1}}}}
\newcommand{\transitiondens}[1]{\ifthenelse{\equal{#1}{0}}{m_0}{m_{#1}}}
\newcommand{\bitransition}[2]{\mathcal{M}^{#1} _{#2}}
\newcommand{\mumeasure}[1]{\mathcal{Q}_{#1}}
\newcommand{\bounded}[1]{\ifthenelse{\equal{#1}{}}{\ensuremath{\mathsf{F} (\mathcal{X})}}{\ensuremath{\mathsf{F} (\mathcal{X}^{\otimes {#1}})}}}
\newcommand{\measurable}[1]{\ifthenelse{\equal{#1}{}}{\ensuremath{\mathsf{F}(\mathcal{X})}}{\ensuremath{\mathsf{F}(\mathcal{X}^{\otimes {#1}})}}}
\newcommand{\additive}[1]{\mathbb{A}_b(\mathcal{X}^{\otimes #1})}
\newcommand{\muest}[2]{\mathcal{Q}^{N,#1} _{#2}}
\newcommand{\backwardTest}[4]{\mathrm{\mathbf{T}}^{#1} _{#2}(#3, #4)}
\newcommand{\backwardT}[3]{\mathrm{\mathbf{T}}_{#1}(#2, #3)}
\newcommand{\predasymptvar}[2]{\mathcal{V}^{\infty}_{\eta, #1} \left(#2\right)}
\newcommand{\jointasymptvar}[2]{\mathcal{V}^{\infty}_{\gamma, #1} (#2)}
\newcommand{\jointasymptvarestim}[2]{\mathcal{V}^{N}_{\gamma, #1} (#2)}
\newcommand{\predasymptvarestim}[2]{\mathcal{V}^{N}_{\eta, #1} (#2)}
\newcommand{\asymptvar}[1]{\mathcal{V}^{\infty} _{#1}}
\newcommand{\asymptvarestim}[2]{\mathcal{V}^{N,#2} _{#1}}
\newcommand{\scdjointasymptvarestim}[2]{\overline{\mathcal{V}}^{N}_{\gamma,#1} (#2)}
\newcommand{\jointestimchan}[2]{\mathcal{V}^{N, \infty}_{#1} (#2)}
\newcommand{\jointestimlee}[2]{\mathcal{V}^{N, \infty}_{#1} (#2)}
\newcommand{\idealasymptvarest}[2]{\Gamma^{#2} _{#1} (h_{0:#1})}
\newcommand{\jointvarestim}[3]{\mathcal{V}^{N, #3}_{\gamma, #1} (#2)}
\newcommand{\tbtasymptvarestim}[2]{\mathcal{\overline{V}}{\vphantom{\mathcal{V}}}^{N,#2} _{#1}}
\newcommand{\scdjointvarestim}[3]{\overline{\mathcal{V}}^{N, #3}_{\gamma, #1} (#2)}
\newcommand{\parisasymptvar}[2]{\mathsf{V}^{N,M} _{#1}}
\newcommand{\asymptvaresttf}[2]{\ensuremath{\widetilde{\Gamma}^{#2} _{#1} (h_{0:#1})}}
% \newcommand{\esssup}[2][]
% {\ifthenelse{\equal{#1}{}}{\left\| #2 \right\|_\infty}{\left\| #2 \right\|^2_{\infty}}}
% \newcommand{\eqdef}{\ensuremath{:=}}
% \newcommand{\eqsp}{}
% \newcommand{\weight}[2]{\tilde{\omega}^{#1} _{#2}}
% \newcommand{\normweight}[2]{\mathcal{W}^{#1} _{#2}}
\newcommand{\normweight}[2]{\omega^{#1} _{#2}}
\newcommand{\particle}[2]{\xi^{#1} _{#2}}
\newcommand{\particleQ}[2]{\mathsf{Q}^N _{#2}(A^{1:N} _{#1}, \rmd \particle{1:N}{#2})}
\newcommand{\condparticleQ}[3]{\mathsf{Q}^{#3, N} _{#1 + 1}(#2 _{#1 + 1};  \rmd \particle{1:N \setminus \{#2 _{#1 + 1}\}}{#1 +1}, A^{1:N} _{#1})}
\newcommand{\smclaw}[1]{\mathrm{P}^N (A^{1:N} _{0:#1-1},\rmd \particle{1:N}{0:#1})}
\newcommand{\condsmclaw}[3]{\mathrm{P}^N _{#3} (#2 _{0:#1};  A^{1:N} _{0:#1 -1},\rmd \particle{1:N \setminus \{#2 _{0:#1}\}}{0:#1})}
\newcommand{\condchi}[1]{\bar{\chi}(#1 _{0}; \rmd \particle{1:N \setminus \{ #1 _0\}}{0})}
\newcommand{\smclawtraj}[2]{\mathrm{P}^N (\rmd \particle{}{0:#1}, A _{0:#1-1}, #2 _{0:#1})}
% \newcommand{\mixture}[3]{
%     \ifthenelse{\equal{#3}{}}{\mathrm{Q} _{#1}(\particle{1:N}{#1 -1}, \rmd \particle{#2}{#1})}{\mathrm{Q}^{\otimes #3} _{#1}(\particle{1:N}{#1}, \rmd \particle{#2}{#1})}}
\newcommand{\ffbsasymptvar}[3]{\mathcal{V}^{#1} _{#2 | #3}}
\newcommand{\parismuest}[2]{\widetilde{\mathcal{Q}}^{N,M} _{#2}}
% \newcommand{\A}[2]{\ifthenelse{\equal{#2}{}}{(\mathbf{A}{\mathbf{\ref{#1})}}}{(\mathbf{A}\mathbf{\ref{#1}:\ref{#2}})}}
\newcommand{\As}[2]{\ifthenelse{\equal{#2}{}}{(\mathbf{A}{\mathbf{\ref*{#1})}}}{(\mathbf{A}\mathbf{\ref*{#1}:\ref*{#2}})}}
\newcommand{\RQ}[1]{(\textbf{Q}{#1})}
\newcommand{\muDDIM}[1]{\mu_{#1}}

%NEO def

\def\param{\theta}
\def\gauss{\Normal}
 \def\elboneq{\mathcal{L}_{\IFIS}}
\def\argmax{\arg \max}
\def\hparam{\theta^*}
\def\Param{\Theta}
\def\logit{\operatorname{logit}}
 \def\flow{\mathbf{T}}
\def\Cat{\operatorname{Cat}}
\def\tU{\tilde{U}}
 \def\mass{\mathrm{M}}
 \def\Normal{\mathrm{N}}
  \providecommand{\assumptionname}{Assumption}
  \providecommand{\corollaryname}{Corollary}
  \providecommand{\lemmaname}{Lemma}
  \providecommand{\propositionname}{Proposition}
  \providecommand{\remarkname}{Remark}
\providecommand{\theoremname}{Theorem}
%\usepackage[disable]{todonotes}

\def\plaw{\operatorname{g}}

\def\simiid{\overset{\operatorname{iid}}{\sim}}
%% math commands go here
\def\IFIS{\ensuremath{\operatorname{NEO}}}
\def\InFiNE{{\small \IFIS}}
\def\NEO{{\small \IFIS}}

\def\MC{\mathrm{MC}}
\def\transfo{\operatorname{T}}
\def\dmid{\left.\middle\|\right.}
\def\rmd{\operatorname{d}\hspace{-2pt}}
\def\Id{\mathbf{Id}}
\def\PP{\mathbb{P}}
\def\QQ{\mathbb{Q}}
% \def\pE{\mathbb{E}}
\def\PVar{\mathrm{Var}}
\def\mcf{\mathcal{F}}
\def\Ind{\mathbb{I}}
\def\ELBO{\operatorname{ELBO}}
\def\rset{\mathbb{R}}
\def\brset{\overline{\mathbb{R}}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}_{>0}}
\def\Ber{\mathrm{Ber}}
\def\dummy{f}
\def\nmeasrho{\tilde{\measrho}}
\def\suppvarpi{\mathbb{S}}
\newcommandx{\Exp}[2][1=]{\ensuremath{\pE_{#1}\left[ #2\right]}}
\def\Var{\operatorname{Var}}
\newcommandx{\marginal}[2][1=]{\ensuremath{\xi^{#2}_{#1}}}

\newcommandx{\margindensm}[2]{m_{#1}^{#2}}
\newcommandx{\margindensmu}[4]{m_{#1}^{#2}(#3|#4)}
\newcommand{\partint}[1]{ \left \lfloor #1 \right \rfloor}

\newcommandx{\margindens}[4][4=]{\ifthenelse{\equal{#3}{}}{q_{#1}^{#4}(#2)}{q_{#1,#3}^{#4}(#2)}}
\newcommandx{\margindensw}[3][3=]{\ifthenelse{\equal{#3}{}}{q_{#1}^{#2}}{q_{#1,#3}^{#2}}}
\newcommand{\Mtrans}[4]{Q_{#1,#4}(#2,#3)}
\newcommand{\Mtransw}[2]{Q_{#1,#2}}
% \newcommand{\chunk}[3]{#1_{#2:#3}}
% \newcommand{\KL}[2]{\operatorname{KL}\left(#1\Vert #2\right)}
\newcommand{\KLLigne}[2]{\operatorname{KL}(#1| #2)}
\def\lowerbound{\mathcal{L}}
\def\lowerboundaux{\mathcal{L}_{\mathrm{aux}}}
\def\tlowerboundaux{\tilde{\mathcal{L}}_{\mathrm{aux}}}
\def\rmd{\mathrm{d}}
\def\bigO{\mathcal{O}}
\def\eqsp{\,}

\def\fwdtransfo{T}
\newcommandx{\fwdtransfoparam}[2]{\fwdtransfo_{#1,#2}}
\def\famtransfo{\mathcal{T}}
\def\invtransfo{\mathring{\fwdtransfo}}
\def\trueflow{\mathsf{T}}

\def\dmhratio{\mathring{\alpha}_{\phi,\tu}}
\def\counting{\mathsf{c}}
% \renewcommand{\sqrt}[1]{#1 ^{1/2}}
\def\msa{\mathsf{A}}
% \def\borel{\mathcal{B}}
\newcommand{\defeq}{\vcentcolon=}
% \newcommand{\eqdef}{=\vcentcolon}

\def\dimE{M}
\def\dimS{D}


\def\eg{\text{e.g.}}



\def\rmb{\mathrm{b}}

\def\mcu{\mathcal{U}}
\def\wrt{w.r.t.}

\def\phibf{\pmb{\phi}}
\def\bfphi{\phibf}

% Operands
\newcommand{\absolute}[1]{\left\vert #1 \right\vert}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\absLigne}[1]{\vert #1 \vert}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathsf{TV}}}
\newcommand{\tvnormEq}[1]{\left \| #1 \right \|_{\mathrm{TV}}}
\newcommandx{\Vnorm}[2][1=V]{\| #2 \|_{#1}}
\newcommandx{\VnormEq}[2][1=V]{\ensuremath{\left\| #2 \right\|_{#1}}}
% \newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
% \newcommandx{\normLigne}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2\Vert^{#1}}}
\newcommand{\crochet}[1]{\left\langle#1 \right\rangle}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\newcommand{\parentheseLigne}[1]{(#1 )}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\newcommand{\parentheseDeuxLigne}[1]{[ #1 ]}
\newcommand{\defEns}[1]{\left\lbrace #1 \right\rbrace }
\newcommand{\defEnsLigne}[1]{\lbrace #1 \rbrace }
\newcommand{\defEnsPoint}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsPointDeux}[1]{\left. #1 \right  \rbrace }
\newcommand{\defEnsL}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsR}[1]{\left. #1 \right  \rbrace }

%\newcommand{\defSystem}[1]{\left\lbrace #1 \right. }

\newcommand{\ps}[2]{\left\langle#1,#2 \right\rangle}
\newcommand{\psLigne}[2]{\langle#1,#2 \rangle}

% Relations
\newcommand{\divid}{\mid}
\newcommand{\ndivide}{\nmid}

% Proba
\newcommand{\proba}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\probaCond}[2]{\mathbb{P}\left( \left. #1  \middle\vert #2 \right.\right)}
\newcommand{\probaLigne}[1]{\mathbb{P}( #1 )}
\newcommandx\probaMarkovTilde[2][2=]
{\ifthenelse{\equal{#2}{}}{{\widetilde{\mathbb{P}}_{#1}}}{\widetilde{\mathbb{P}}_{#1}\left[ #2\right]}}
\newcommand{\probaMarkov}[2]{\mathbb{P}_{#1}\left[ #2\right]}
\newcommand{\expe}[1]{\pE \left[ #1 \right]}
\newcommand{\expeExpo}[2]{\pE^{#1} \left[ #2 \right]}
\newcommand{\expeLigne}[1]{\pE [ #1 ]}
\newcommand{\expeLine}[1]{\pE [ #1 ]}
\newcommand{\expeMarkov}[2]{\pE_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovLigne}[2]{\pE_{#1} [ #2 ]}
\newcommand{\expeMarkovExpo}[3]{\pE_{#1}^{#2} \left[ #3 \right]}
\newcommand{\probaMarkovTildeDeux}[2]{\widetilde{\mathbb{P}}_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovTilde}[2]{\widetilde{\pE}_{#1} \left[ #2 \right]}
\newcommand{\tmestep}[1]{{t_{#1}}}
% Environments

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}



%fleche limite
\newcommand{\flecheLimite}{\underset{n\to+\infty}{\longrightarrow}}
\newcommand{\flecheLimiteOption}[2]{\underset{#1\to#2}{\longrightarrow}}
\newcommand{\flecheLimiteHaut}{\overset{n\to+\infty}{\longrightarrow}}


%notation infini
\newcommand{\plusinfty}{+\infty}

%notation egale
\newcommand{\egale}[1]{\ensuremath{\underset{#1}{=}}}

%plusieurs ligne indice
%\sum\limits_{\substack{i=0 \\ i \neq i_0}}^{n}{A_



\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


\newcommand{\hilbert}{\mathcal{H}}


\def\ie{\textit{i.e.}}
%\def\as{almost surely}
\def\cadlag{càdlàg}
\def\eqsp{\;}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}
\renewcommand{\iint}[2]{\left\lbrace #1,\ldots,#2\right\rbrace}
\newcommand{\iintLigne}[2]{\lbrace #1,\ldots,#2\rbrace}


\def\primr{f_r}
\def\primrO{f_{r_0}}



% \newcommand{\1}{\mathbbm{1}}
% \newcommand{\indi}[1]{\1_{#1}}
\newcommand{\indiacc}[1]{\mathbbm{1}_{\{ #1   \}}}
% \newcommandx{\weight}[2][2=n]{\omega_{#1,#2}^N}
\newcommand{\loi}{\mathcal{L}}
\newcommand{\boule}[2]{\operatorname{B}(#1,#2)}
\newcommand{\ball}[2]{\operatorname{B}(#1,#2)}
\newcommand{\boulefermee}[2]{\overline{\mathrm{B}}(#1,#2)}
\newcommand{\diameter}{\operatorname{diam}}
\newcommand{\deta}{d_{\eta}}
% \def\divergence{\operatorname{div}}
\def\TV{\mathrm{TV}}
\def\Tvarpi{T_\varpi}
\newcommand{\tme}[1]{{t_{#1}}}
% \def\argmax{ \arg \max}
% \def\argmin{ \arg \min}



 \newcommand{\alaini}[1]{\todo[color=black!20,inline]{{\bf AD:} #1}}
%   \newcommand{\alain}[1]{\todo[color=black!20]{{\bf AD:} #1}}
% \newcommand{\tcb}[1]{\textcolor{blue}{#1}}
 \newcommand{\eric}[1]{\todo[color=red!20]{{\bf Eric:} #1}}
  \newcommand{\xian}[1]{\todo[color=orange!30]{{\bf Xian:} #1}}
  \newcommand{\achille}[1]{\todo[color=blue!30]{{\bf AT:} #1}}

\def\as{almost surely}
\def\dist{\operatorname{dist}}

\newcommand{\seq}[3]{(#1) _{#2} ^{#3}}
\newcommandx\sequence[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2}, \eqsp #2 \in #3 \}}}}
\newcommandx\sequenceD[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{( #1)_{ #2 \in #3} }}}

\newcommandx{\sequencen}[2][2=n\in\N]{\ensuremath{\{ #1_n, \eqsp #2 \}}}
\newcommandx\sequenceDouble[4][3=,4=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ (#1_{#3},#2_{#3}) \}}}{\ensuremath{\{  (#1_{#3},#2_{#3}), \eqsp #3 \in #4 \}}}}
\newcommandx{\sequencenDouble}[3][3=n\in\N]{\ensuremath{\{ (#1_{n},#2_{n}), \eqsp #3 \}}}


\def\iid{i.i.d.}
\def\ifof{if and only if}
% \def\eg{e.g.}




\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}


\def\momentNoise{\mathrm{m}}
\def\bfe{\mathbf{e}}

\def\bfv{\mathbf{v}}
\def\ebf{\mathbf{e}}
\def\vbf{\mathbf{v}}


\def\Id{\operatorname{Id}}

\def\tildetheta{\tilde{\theta}}

\def\calC{\mathcal{C}}

\def\varphibf{\operatorname{g}}
\newcommandx{\CPE}[3][1=]{{\mathbb E}_{#1}\left[\left. #2 \middle \vert #3 \right. \right]} %%%% esperance conditionnelle
\newcommandx{\CPVar}[3][1=]{\mathrm{Var}^{#3}_{#1}\left\{ #2 \right\}}
\newcommand{\CPP}[3][]
{\ifthenelse{\equal{#1}{}}{{\mathbb P}\left(\left. #2 \, \right| #3 \right)}{{\mathbb P}_{#1}\left(\left. #2 \, \right | #3 \right)}}

\def\Ascr{\mathscr{A}}
\def\scrA{\mathscr{A}}
\def\scrB{\mcbb}
\def\scrC{\mathscr{C}}

\def\barL{\bar{L}}

\def\YL{\mathbf{Y}}
\def\XEM{X}
\def\steps{\gamma}
\def\measSet{\mathbb{M}}

\newcommand\Ent[2]{\mathrm{Ent}_{#1}\left(#2\right)}
\newcommandx{\osc}[2][1=]{\mathrm{osc}_{#1}(#2)}

\def\Ybar{\bar{Y}}
\def\Id{\operatorname{Id}}
\def\IdM{\operatorname{I}_d}
\newcommand\EntDeux[2]{\Ent_{#1}\left[#2 \right]}
\def\Ltwo{\mathrm{L}^2}
\def\Lone{\mathrm{L}^1}
\newcommand\densityPi[1]{\frac{\rmd #1}{\rmd \pi}}
\newcommand\densityPiLigne[1]{\rmd #1 /\rmd \pi}
\newcommand\density[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand\densityLigne[2]{\rmd #1/\rmd #2}

\def\V{V}
\def\VD{V}
\def\Vsp{V^{\sphere^d}_{\b,\beta}}
\def\Vr{V^{\rset^d}_{\b,\c,\beta}}

\def\Prset{P^{\rset^d}}
\def\Psphere{P^{\sphere^d}}

\def\n{\mathrm{n}}
\def\Vpsi{\psi}
\def\Vkappa{\kappa}
\def\Vkappat{\tilde{\kappa}}
\def\Vchi{\chi}
\def\Vchit{\tilde{\chi}}
\def\Vphi{\phi}
\def\Vrho{\rho}
\def\psiV{\Vpsi}
\def\rhoV{\Vrho}
\def\phiV{\Vphi}
\def\fV{f}
\def\Vf{\fV}
\def\kappaVt{\tilde{\Vkappa}}
\def\kappaV{\Vkappa}
\def\chiV{\Vchi}
\def\chiVt{\Vchit}


\def\a{a}
\def\b{b}
\def\c{c}
\def\e{e}
\def\rU{\mathrm{r}}

\def\domain{\mathrm{D}}

\def\martfg{M^{f,g}}
\newcommand\Ddir[1]{D_{#1}}
\newcommand\maxplus[1]{\parenthese{#1}_+}
\def\Refl{\mathrm{R}}
\def\phibf{\pmb{\phi}}
\def\Gammabf{\mathbf{\Gamma}}


%\def\transpose{\operatorname{T}}
\def\transpose{\intercal}
\def\v{v}
\def\w{w}
\def\y{y}
\def\z{z}
%%%% bar

\def\bb{\bar{b}}
\def\bgamma{\bar{\gamma}}
\def\bU{\bar{U}}
\def\Ub{\bU}
\def\lambdab{\bar{\lambda}}
\def\blambdab{\bar{\lambda}}
\def\bv{\bar{v}}
\def\vb{\bv}
\def\yb{\bar{y}}
\def\by{\yb}
\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\taub{\bar{\tau}}

\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}

\def\pib{\bar{\pi}}
\def\bpi{\pib}

\def\S{S}
\def\target{\pi}
\def\proposal{\rho}
\def\weightfunc{\tilde{w}}
\newcommand{\chunku}[3]{#1^{#2:#3}}
\newcommand{\chunkl}[3]{#1_{#2:#3}}
\newcommand{\chunkul}[5]{#1_{#2:#3}^{#4:#5}}
\newcommand{\chunkum}[4]{#1^{#2:#3 \setminus \{#4\}}}
\newcommand{\chunkulm}[6]{#1_{#2:#3}^{#4:#5 \setminus \{#4\}}}
\def\tmidIR{\ensuremath{\operatorname{i-SIR}}}
%%%%
% \tilde

\def\tr{\tilde{r}}
\def\tc{\tilde{c}}
\def\tmsk{\tilde{\msk}}
\def\tW{\tilde{W}}
\def\tvarsigma{\tilde{\varsigma}}
% \def\tv{\tilde{v}}
\def\vt{\tv}
\def\yt{\tilde{y}}
\def\ty{\yt}
\def\Mt{\tilde{M}}
\def\tM{\Mt}

\def\tx{\tilde{x}}
\def\xt{\tx}
\def\Xt{\tilde{X}}
\def\Yt{\tilde{Y}}
\def\Gt{\tilde{G}}
\def\Et{\tilde{E}}
\def\Tt{\tilde{T}}
\def\St{\tilde{S}}
\def\taut{\tilde{\tau}}

\def\tX{\tilde{X}}
\def\tY{\tilde{Y}}
\def\tG{\tilde{G}}
\def\tE{\tilde{E}}
\def\tT{\tilde{T}}
\def\tS{\tilde{S}}
\def\ttau{\tilde{\tau}}
\def\teta{\tilde{\eta}}
\newcommand{\ttheta}{\tilde{\theta}}


%%%%%
% \bar
\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\Sb{\bar{S}}
\def\taub{\bar{\tau}}
\def\Hb{\bar{H}}
\def\Nb{\bar{N}}


\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}
\def\bS{\bar{S}}
\def\bH{\bar{H}}
\def\bN{\bar{N}}

%%%%%%%%

\def\mgU{\mathrm{m}_{\nabla U}}
\def\MintDrift{I}
\def\CU{C_U}
\def\RU{R_1}
\def\RV{R}
\def\Reps{R_{\epsilon}}
\def\Resp{\Reps}
\def\veps{\varepsilon}
\def\sphere{\mss}

%\def\suppvarpi{\zset}
\def\bound{M_{\transfo}^{\varpi}}
\def\nablaUt{\overline{\nabla U}}
\def\measureSphere{\nu^d}
\def\wcont{w_t^\mathrm{c}}
\def\etaU{\eta}
\def\epsilonU{\epsilon}
\def\rhoTcont{\rhoT^{\operatorname{c}}}
\def\NEIS{\ensuremath{\operatorname{NEIS}}}
\def\Jac{\mathbf{J}}
\newcommand{\JacOp}[1]{\Jac_{#1}}
\def\jac{\operatorname{Jac}}
\def\sign{\operatorname{sign}}
\def\rate{\lambda_{\mathrm{r}}}
\newcommand{\intentier}[2]{[#1:#2]}
\newcommand{\intentierU}[1]{[#1]}
%\newcommand{\intentier}[2]{#1:#2}
\def\measrho{\boldsymbol{\rho}}
\def\rmi{\mathrm{I}}
\def\ne{\mathrm{ne}}
\def\const{\operatorname{Z}}
\def\estConst{\widehat{\const}^{\varpi}}
\newcommand{\estConstC}[1]{\widehat{\const}^{\varpi}_{#1}}
\newcommand{\estConstCphi}[2]{\widehat{\const}_{#1}^{#2}}
\newcommand{\hatpi}[1]{\hat{\pi}_{#1}}
%\def\hatpi{\hat{\pi}}
\def\measpi{\boldsymbol{\pi}}
\def\measprop{\boldsymbol{\rho}}
\def\measq{\boldsymbol{q}}

\def\trace{\operatorname{tr}}
\def\sigmaS{\sigma^2}
\def\adj{\operatorname{adj}}
\newcommand{\ensemble}[2]{\left\{#1\,:\eqsp #2\right\}}
\newcommand{\ensembleLigne}[2]{\{#1\,:\eqsp #2\}}
\newcommand{\set}[2]{\ensemble{#1}{#2}}

\def\rmD{\mathrm{D}}%%rmd déjà pris
\def\mrd{\mathrm{D}}
\def\mrc{\mathrm{C}}

% \def\diag{\Delta_{\rset^d}}

\def\lyap{V}
\newcommand\coupling[2]{\Gamma(\mu,\nu)}
\def\supp{\mathrm{supp}}
\def\tpi{\tilde{\pi}}
\def\tPi{\tilde{\Pi}}
\newcommand\adh[1]{\overline{#1}}

\def\ACb{\mathrm{AC}_{\mathrm{b}}}

\def\opK{\mathrm{K}}

\newcommand{\fracm}[2]{\left. #1 \middle / #2 \right.}

\newcommand{\complementary}{\mathrm{c}}

\def\poty{H}
\def\diam{\mathrm{diam}}
\def\talpha{\tilde{\alpha}}
\def\Leb{\mathrm{Leb}}
\newcommand{\iintD}[2]{\{#1,\ldots,#2\}}
\def\interior{\mathrm{int}}
\def\iff{ if and only if }

\def\vareps{\varepsilon}
\def\varespilon{\varepsilon}
\def\si{\text{ if } }
\def\projd{\operatorname{proj}^{\msd}}
\def\Phibf{\mathbf{\Phi}}

\def\RKer{R_{\gamma}}

\def\VEa{V}
\def\KUa{K}
\def\vol{\operatorname{Vol}}

\newcommand*\Let[1]{\State #1 }

\def\mU{\mathrm{m}}

\newcommand\fraca[2]{(#1)/(#2)}

\def\ccur{\mathtt{c}}
\def\Ve{V_{\rme}}
\def\Rad{\operatorname{Rad}}
%%% mathsf
\def\msi{\mathsf{I}}
\def\msw{\mathsf{W}}
\def\msa{\mathsf{A}}
\def\msd{\mathsf{D}}
\def\msk{\mathsf{K}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\msat{\tilde{\mathsf{A}}}
\def\msb{\mathsf{B}}
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{O}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\tmsu{{\mathsf{U}}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
\def\msx{\mathsf{X}}
\def\msy{\mathsf{Y}}

\def\msphi{\mathsf{\Phi}}

%% mathcal
\def\mca{\mathcal{A}}
\def\mcl{\mathcal{L}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcbb{\mathcal{B}}  %%% \mcb est déjà pris
\def\mcc{\mathcal{C}}
\def\mcy{\mathcal{Y}}
\def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}

%% mathbb

\def\rset{\mathbb{R}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^*}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}


%%%% mathrm


\def\rmP{\mathrm{P}}
\def\rmQ{\mathrm{Q}}
\def\rml{\mathrm{L}}
\def\rmR{\mathrm{R}}
\def\rmS{\mathrm{S}}
\def\rmT{\mathrm{T}}
\def\rmM{\mathrm{M}}
\def\Prm{\mathrm{P}}
\def\rmb{\mathrm{b}}
\def\mrb{\mathrm{b}}
\def\rmd{\mathrm{d}}
\def\rmZ{\mathrm{Z}}
\def\mrd{\mathrm{d}}
\def\mre{\mathrm{e}}
\def\rme{\mathrm{e}}
\def\rmn{\mathrm{n}}
\def\mrn{\mathrm{n}}
\def\mrc{\mathrm{C}}
\def\mrcc{\mathrm{c}}
\def\rmc{\mathrm{C}}
\def\rmcc{\mathrm{c}}
\def\rma{\mathrm{a}}
\def\mra{\mathrm{a}}
\def\rmC{\mathrm{C}}

\def\tu{u}
\def\FamilyVar{\mathcal{Q}}
\def\RWM{\scriptscriptstyle{\operatorname{RWM}}}
\def\MALA{{\scriptscriptstyle{\operatorname{MALA}}}}
\def\MH{\mathsf{MH}}
\def\stephmc{\upgamma}
\def\Sigmahmc{\Sigma}
\def\densgauss{\varphibf}
\def\LF{\mathsf{LF}}
\def\Refresh{\mathsf{ref}}

% \newcommand{\card}[1]{\vert #1\vert}
\def\tz{\tilde{z}}

\def\Idd{\mathrm{Id}}
\def\likeratio{\kappa}
\def\minor{\varepsilon}

\newcommandx{\estpiNaive}[3][1=g,2=N,3=f]{\hat{\pi}_{#1}^{#2}(#3)}
\def\bmeaspi{\bar{\measpi}}
\def\bmeasq{\bar{\measq}}

\def\rhobf{\measrho}

\def\bfm{\mathbf{m}}

\newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
\newcommandx{\normLigne}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2 \Vert^{#1}}}
\def\gaussianD{\operatorname{g}}
\def\rhoT{\rho_{\transfo}}
\def\constT{\const_{\transfo}}
\def\pdf{p.d.f.}
% \def\wrt{with respect to}

\def\oQ{\operatorname{Q}}
\def\oP{\operatorname{P}}


\def\infineIS{I^{\NEO}_{\varpi,N}}
\def\infineISh{I^{\NEO}_{\varpi,N,h}}
\def\infineSNIS{J^{\NEO}_{\varpi,N}}
\def\txts{\textstyle}
\def\support{\mathrm{support}}
\def\varpic{\varpi^{\mathrm{c}}}
\def\final{n}

\def\target{\pi}
\def\statespace{\mathbb{X}}
% \def\xsp{\mathsf{X}}
\def\unit{\mathbf{1}}
\def\zero{\mathbf{0}}
\def\identity{\mathbf{I}}
\def\Utarget{\widetilde{\pi}}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\rmd{\mathrm{d}}
\def\tribu{\mathcal{B}(\mathcal{X})}
\def\param{\theta}
\def\paramspace{\Theta}
\def\transform{\mathrm{T}}
\def\indic{\mathbbm{1}}
\def\kernel{\mathrm{K}}
\def\pE{\mathbb{E}}
\def\pV{\mathbb{V}}
\def\transitionker{K_\target}
\def\gauss{\mathcal{N}}
% \def\Q{\mathrm{Q}}
\def\ula{\texttt{ULA}}
\def\mala{\texttt{MALA}}
\def\emalg{\texttt{EM}}
\def\rnvp{\texttt{RNVP}}
\def\P{\mu}
\def\heavy{h}
\def\1{\mathbbm{1}}
\def\probmeasures{\mathsf{M}_1}
\def\probmeasuresac{\mathsf{M}_{\target}}
\def\MCMCker{\mathrm{M}_\target}
\def\const{\mathcal{Z}}
\def\ratioQ{\mathcal{R}_\beta}
\def\bigo{\mathcal{O}}
\def\dkl{\mathbb{D}_{\mathrm{KL}}}
\def\distr{\mu}
\def\frakconst{\mathcal{Z}}
\def\student{\mathrm{Student}}
\def\paramfamily{\mathsf{F}_{\Theta}}
\def\kl{\mathrm{KL}}
\def\gm{\mathsf{GM}}
\def\rnvp{\mathtt{RNVP}}
\def\dontread{\textbf{\textcolor{red}{en chantier} }}
\def\localker{L_\target}
\def\pow{\varepsilon}
\def\half{\frac{1}{2}}
\def\EMC{\texttt{EM2C}}
\def\tbf{\textcolor{purple}{(To be finished.)}}
\def\projtarg{\target_*}
\def\renyiset{\mathsf{R}_{2,3}}
\def\infrenyiset{\mathsf{R}_\infty}
\def\Fmap{\mathcal{F}}
\def\Linf{\mathrm{L}^\infty}
\def\emFmap{\mathcal{F}_{\mathsf{em}}}
\def\eFmap{\mathcal{F}_{\mathsf{e}}}
\def\ulaker{\mathsf{R} _\gamma}
\def\lsconst{C_{\mathrm{LS}}}

\newcommand{\supnorm}[1]{\| #1 \|_\infty}
\newcommand{\skrenyi}[2]{\widetilde{\mathcal{R}}_{\target}(#1 \parallel #2)}
\newcommand{\ulaiterate}[1]{\iterate{#1}^{\mathsf{R}}}
\newcommand{\Fmc}[1]{\zeta^N _{#1}}
\newcommand{\constmu}[1]{\mathcal{Z}_{\iterate{#1}}}
\newcommand{\constmuK}[1]{\mathcal{Z}_{\iterate{#1} \transitionker}}
\newcommand{\mciterate}[1]{\mu^n _{#1}}
\newcommand{\gradinterpo}[1]{\overline{\nabla U}_{#1}}
\newcommand{\esssup}[1]{\mathrm{ess}\sup_{\lambda}}
\newcommand{\approxit}[1]{\mu_{\param _{#1}}}
\newcommand{\propo}[1]{\vartheta_{#1}}
\newcommand{\rnikodd}[3]{\frac{#1(#3)}{#2(#3)}}
% \newcommand{\rnikod}[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand{\proposalmap}{\vartheta}
\newcommand{\iterate}[1]{\mu_{#1}}
\newcommand{\iter}[3]{\Psi_{#1, #3}(#2)}
\newcommand{\tditerate}[1]{\tilde{\mu}_{#1}}
\newcommand{\sqmapping}[2]{
        \ifthenelse{\equal{#1}{}}
        {
            \mathcal{R}^{\pow,2} _{ #2}
            }
        {
            \mathcal{R}^{\pow_{#1}, 2} _ #2
            }}
\newcommand{\mapping}[2]{
        \ifthenelse{\equal{#1}{}}
        {
            \Psi^{\pow} _{ #2}
            }
        {
            \Psi^{\pow_{#1}} _{#2}
            }}
\newcommandx{\denoiser}[2][2=\param]{D^{#2} _{#1}}
\newcommandx{\score}[2][2=\param]{s^{#2} _{#1}}
\newcommandx{\scores}[2][2=\param]{s^{#2^{\star}} _{#1}}
\newcommand{\mixture}[1]{\mathcal{M}^\pow _{#1}}
% \newcommand{\uweight}[2]{\omega^{#1} _{#2}}
% \newcommand{\tv}[1]{\left\|#1\right\|_{\mathsf{TV}}}
\newcommand{\hatC}[1]{\widehat{\mathcal{C}}_{\target,#1}}
\newcommand{\urbetaK}[1]{\widetilde{\mathcal{R}}_{\beta, #1}}
\newcommand{\rbetaK}[1]{\mathcal{R}_{\beta, #1}}
\newcommand{\rbetaKstr}[1]{\mathfrak{R}_{\beta, #1}}
\newcommand{\ratio}[2]{\mathcal{R}_{#1}[#2]}
\newcommand{\ptheta}[1]{\mathrm{P}_{\param{#1}}}
% \newcommand{\particle}[2]{\xi^{#1} _{#2}}
\newcommand{\Tparticle}[2]{\widetilde{\xi}^{#1} _{#2}}
\newcommand{\paramiterate}[1]{\bar\mu_{\param#1}}
% \newcommand{\eqdef}{\ensuremath{:=}}
% \newcommand{\eqsp}{}
\newcommand{\piterate}[2]{\ifthenelse{\equal{#2}{}}{\hat\mu_{\param, #1}}{\hat\mu_{\param#2, #1}}}
% \newcommand{\weight}[1]{\omega_{#1}}
% \newcommand{\normweight}[2]{\mathcal{W}^{#1} _{#2}}
\newcommand{\borelians}[1]{\mathcal{B}(\mathbb{R}^{#1})}
\newcommand{\targetrestr}[1]{\target_{| #1}}
% \newcommand{\divergence}[3]{\mathcal{R}_{#1}(#2 \parallel #3)}
% \newcommand{\kldivergence}[2]{\mathsf{KL}(#1 \parallel #2)}
\newcommand{\pushptheta}[2]{#1_{\#} \ptheta{#2}}
\newcommand{\C}[1]{\mathcal{C}_{\target, #1}}
\newcommand{\sumC}[1]{\mathcal{S} _{#1}}
\newcommand{\UsumC}[1]{\widetilde{\mathcal{S}} _{#1}}
\newcommand{\hatsumC}[2]{\widehat{\mathcal{S}}^{#2} _{#1}}
\newcommand{\hatUsumC}[2]{\widehat{\mathsf{S}}^{\mathrm{u} #2} _{#1}}
\newcommand{\A}[2]{\ifthenelse{\equal{#2}{}}{(\textbf{A}{\textbf{\ref{#1})}}}{(\textbf{A}\textbf{\ref{#1}-\ref{#2}})}}
\newcommand{\assp}[1]{(\textbf{A}\textbf{#1})}
\newcommand{\average}[1]{\mathcal{A}_{\beta, #1}}
\newcommand{\law}[1]{\mathsf{Law}(#1)}

%mcgdiff notations

\def\obs{y}
\newcommand{\iobs}[1]{{\obs_\tstep{#1}}}
\def\nsteps{S}
\def\cov{\mathbb{C}\mathrm{ov}}
\def\covobs{\Sigma_\obs}
\def\obsrv{Y}
\def\rmd{\mathrm{d}}
\def\pP{\mathbb{P}}
\def\noise{\varepsilon}
\def\noiserv{Z}
\def\pE{\mathbb{E}}
\def\pV{\mathbb{V}}
\def\ltrstate{x}
% \def\eqdef{:=}
\def\baseset{\Omega}
\def\basesigma{\mathcal{F}}
\def\baseprob{\mathbb{P}}
\def\eqsp{\,}
\def\1{\mathbbm{1}}
\def\dimx{{d_{x}}}
\def\dimz{d_z}
\def\dimy{d_y}
% \def\dimtr{{\smash{\overline{d}}}}
\def\dimtr{\mathsf{t}}
\newcommand{\numsqrt}[1]{\smash{#1}^{1/2}}
\def\dimorig{{d_{\mathbf{y}}}}
% \def\dimb{\smash{\underline{d}}}
\def\dimb{\mathsf{b}}
\def\trmeas{Y}
\def\ltrmeas{y}
\def\ormeas{\mathbf{Y}}
\def\lmeas{\mathbf{y}}
\def\revmeas{\overleftarrow{Y}}
\def\state{\mathbf{X}}
\def\diffltrmeas{\mathsf{\ltrmeas}}
\def\trstate{X}
\def\rset{\mathbb{R}}
\def\nset{\mathbb{N}}
\def\nsetpos{\mathbb{N}_*}
\def\idm{\operatorname{I}}
\def\nlessc{\m{J}^0}
\def\top{\mathsf{t}}
\def\bot{\mathsf{b}}
\def\nyc{\m{J}}
\newcommand{\m}[1]{\operatorname{#1}}
\newcommand{\cat}[2]{{#1}^{\scriptscriptstyle\frown}#2}
\newcommand{\vect}[1]{\mathbf{#1}}
% \DeclareMathOperator*{\argmin}{argmin}
\def\gauss{\mathcal{N}}
\def\noise{\varepsilon}
\def\R{\mathbb{R}}
\def\bV{\mathbf{V}}
% \DeclareMathOperator*{\argmax}{argmax}
\def\bY{\mathbf{Y}}
\def\stateperp{\mathbf{x}^\perp}
\def\stateperp{\bm{\xi}^\perp}
\def\invX{\xi}
\def\perpstate{\bm{\xi}}
\def\parallelstate{\bm{\zeta}}
% \def\datadistr{\pi_*}
\def\param{\theta}
\def\sigalgebra{\mathcal{B}}
\def\normpdf{\mathcal{N}}
% \def\normpdf{\phi}
\def\normdist{\mathcal{N}}
\def\normconst{\mathcal{Z}}
\def\sumweights{\Omega}
\def\boundedfunc{\mathsf{F}}
\def\bigo{\mathcal{O}}
\def\eigSigmay{\sigma^y}
\def\eigA{\sigma^A}
\def\id{\mathbf{I}}
\def\categorical{\mathrm{Categorical}}
\def\ouralgorithm{\algo}
\def\motif{\mathcal{M}}
\def\scaffold{\mathcal{S}}
% \newcommand{\card}[1]{|#1|}
\newcommand{\floor}[1]{{\lfloor #1 \rfloor}}
\newcommand{\eigsigy}[1]{\sigma_{y, #1}}
\newcommand{\twodvect}[2]{(#1, #2)}
\newcommand{\xblock}[2]{x^{B_{#2}} _{#1}}
\newcommand{\filtration}[1]{\mathcal{F}_{#1}}
\newcommand{\fwdker}[3]{\overrightarrow{\mathbf{B}}_{#1}(#2 #3)}
% \newcommand{\uweight}[2]{\widetilde{\omega}^{#1} _{#2}}
% \newcommand{\weight}[2]{\omega^{#1} _{#2}}
\newcommand{\wratio}[3]{\frac{\tilde{\omega}^{#1} _{#2}(#3)}{\Omega^N _{#2}}}
% \newcommand{\kldivergence}[2]{\mathsf{KL}(#1 \parallel #2)}
\def\prtcl{\xi}
\def\tparticle{\smash{\overline{\prtcl}}}
\def\bparticle{\smash{\underline{\prtcl}}}
\newcommand{\iparticle}[2]{x^{#1} _{#2}}
\newcommand{\mset}[2]{\R^{#1 \times #2}}
\newcommand{\X}[1]{X_{#1}}
% \newcommand{\statevar}[1]{\ifthenelse{\equal{#1}{}}{\mathbf{x}}{\mathbf{x}_{#1}}}
\newcommand{\statevar}[1]{\mathbf{x}_{#1}}
% \newcommand{\statevar}[1]{\ifthenelse{\equal{#1}{1}}{\mathbf{x}}{\mathbf{x}_{#1}}}
% \newcommand{\statevar}[1]{\mathbf{x}_{#1}}
\newcommand{\Y}[1]{Y_{#1}}
\newcommand{\revX}[1]{\overset{{}_{\leftarrow}}{X} _{#1}}
\newcommand{\revY}[1]{Y_{#1}}
\newcommand{\W}[1]{W_{#1}}
\newcommand{\condprob}[2]{\baseprob\left(#1|#2\right)}
% \newcommand{\scorenet}[3]{\mathbf{s}_{#1}(#2, #3)}
\newcommand{\zerom}[2]{\mathbf{0}_{#1, #2}}
\def\noisestd{\sigma}
\def\tbw{...}
\def\orthdatadistr{\tilde{\pi}_{*}}
\newcommandx{\acp}[2][2=]{\ifthenelse{\equal{#2}{}}{\alpha_{#1}}{\alpha_{#1:#2}}}
\newcommand{\fwsigma}[2]{\sigma_{#1,#2}}
%  \newcommand{\eric}[1]{\todo[color=blue!20]{{\bf E:} #1}}
 \newcommand{\erici}[1]{\todo[inline,color=blue!20]{{\bf E:} #1}}
% \newcommand\gabriel[1]{\todo[color=green!20]{{\bf G:} #1}}
% \newcommand\yazid[1]{\todo[color=red!20]{{\bf Y:} #1}}
\newcommand\syl[1]{\todo[color=red!60]{{\bf Syl:} #1}}
\newcommandx{\xpred}[2][2=]{\boldsymbol{\chi}^{#2} _{#1}}
\newcommandx{\bottomxpred}[2][2=]{\underline{\boldsymbol{\chi}}^{#2} _{#1}}
\newcommandx{\topxpred}[2][2=]{\overline{\boldsymbol{\chi}}^{#2} _{#1}}
\newcommand{\ndist}[2]{\mathcal{N}(#1, #2)}
\newcommand{\soset}[1]{\operatorname{SO}(#1)}
\newcommand{\tstatevar}[1]{\overline{\mathbf{x}} _{#1}}
\newcommand{\bstatevar}[1]{\underline{\mathbf{x}} _{#1}}
\newcommand{\tstate}[1]{\overline{\state} _{#1}}
\newcommand{\bstate}[1]{\underline{\state} _{#1}}
\newcommand{\tcr}[1]{\textcolor{red}{#1}}
% \newcommand{\prior}[1]{p_{#1}}
% \newcommand{\proposal}[2]{p_{#1, #2}}
\newcommand{\predstartprop}[2]{f_{#2}(#1)}
\newcommand{\epsprop}[2]{\ifthenelse{\equal{#1}{}}{\mathbf{e}^{#2}}{\mathbf{e}^{#2} (#1)}}
\newcommand{\vecidx}[3]{#1 _{#2}[#3]}
\newcommand{\expec}[2]{\mathbb{E}_{ #1}\left[#2\right]}
\newcommand{\realrevbridge}[3]{\ifthenelse{\equal{#2}{}}{\mathsf{q} _{#1}}{\mathsf{q} _{#1}(#3|#2)}}
\newcommand{\revbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{{q}}^{\sigma} _{#1}}{\smash{{q}}^{\sigma} _{#1}(#3|#2)}}
\newcommand{\idxrevbridge}[4]{\ifthenelse{\equal{#2}{}}{\smash{{q}}^{\sigma, #4} _{#1}}{\smash{{q}}^{\sigma, #4} _{#1}(#3|#2)}}
\newcommand{\trevbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{\overline{q}}^{\sigma} _{#1}}{\smash{\overline{q}}^{\sigma} _{#1}(#3|#2)}}
\newcommand{\brevbridge}[3]{\ifthenelse{\equal{#2}{}}{\underline{q}^{\sigma} _{#1}}{\underline{q}^{\sigma} _{#1}(#3|#2)}}
% \newcommand{\realrevbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{\overset{{}_{\leftarrow}}{q}^{\sigma_*}} _{#1}}{\smash{\overset{{}_{\leftarrow}}{q}}^{\sigma_*} _{#1}(#3|#2)}}
% \newcommand{\proposal}[2]{\overleftarrow{q}_{#1,#2}}
\newcommand{\bwproposal}[1]{\overleftarrow{Q}^{#1}}
\newcommand{\ouproposal}[1]{\overrightarrow{P}^{#1}}
\newcommand{\bridge}[4]{{\ifthenelse{\equal{#3}{}}{p^{#2} _{#1}}{p^{#2} _{#1}(#3, #4)}}}
\newcommand{\outrans}[3]{\ifthenelse{\equal{#2}{}}{\overrightarrow{m}_{#1}}{\overrightarrow{m}_{#1}(#2, #3)}}
% \newcommand{\bw }[4]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{m}^{#1}} _{#2}}{\smash{\overset{{}_{\leftarrow}}{m}}^{#1} _{#2}(#4|#3)}}
\newcommandx{\bw }[4][4=]{\ifthenelse{\equal{#3}{}}{q^{#4} _{#1}}{q^{#4} _{#1}(#3|#2)}}
\newcommandx{\fw}[4][4=]{\ifthenelse{\equal{#3}{}}{q^{#4} _{#1}}{q^{#4} _{#1}(#3|#2)}}
\newcommandx{\rbwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{q}^{#4} _{#1}}{\smash{q}^{#4} _{#1}(#3|#2)}}
\newcommandx{\pbwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\hat{p}^{#4} _{#1}}{\hat{p}^{#4} _{#1}(#3|#2)}}
\newcommandx{\abwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{p}^{#4} _{#1}}{\smash{p}^{#4} _{#1}(#3|#2)}}
\newcommandx{\pibw}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\target}^{#4} _{#1}}{\smash{\target}^{#4} _{#1}(#3|#2)}}
\newcommandx{\hbwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\hat{q}}^{#4} _{#1}}{\smash{\hat{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\cabwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{q}^{#4} _{#1}}{\smash{q}^{#4} _{#1}(#3|#2)}}
\newcommandx{\aabwker}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\tilde{q}}^{#4} _{#1}}{\smash{\tilde{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\vbwker}[4][4=\vparam]{\ifthenelse{\equal{#3}{}}{\pi^{#4} _{#1}}{\pi^{#4} _{#1}(#3|#2)}}
\newcommandx{\hpibw}[4][4=\ell]{\ifthenelse{\equal{#3}{}}{\smash{\hat\pi^{#4} _{#1}}}{\smash{\hat\pi^{#4} _{#1}(#3|#2)}}}
\newcommandx{\hmrg}[2][2=\ell]{\smash{\hat\pi^{#2} _{#1}}}
\newcommandx{\cbwtrans}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\Pbwtrans}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{P}}^{#4} _{#1}}{\smash{\overset{{}_{\leftarrow}}{P}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\condbw}[4][4=]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}}{\smash{\overset{{}_{\leftarrow}}{q}}^{#4} _{#1}(#3|#2)}}
\newcommandx{\fwtrans}[4][4=]{\ifthenelse{\equal{#2}{}}{q_{#1}}{q _{#1}(#3|#2)}}
\newcommandx{\cbwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{q^{#3} _{#1}}{q^{#3}_{#1}(#2)}}
\newcommandx{\bwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{p^{#3} _{#1}}{p^{#3}_{#1}(#2)}}
\newcommand{\bwoptmarg}[3]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{{\mathfrak{m}}}}^{#2} _{#1}}{\smash{\overset{{}_{\leftarrow}}{{\mathfrak{m}}}}^{#2} _{#1}(#3)}}
\newcommandx{\fwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{q^{#3} _{#1}}{q^{#3} _{#1}(#2)}}
\newcommandx{\cfwmarg}[3][3=]{\ifthenelse{\equal{#2}{}}{q^{#3} _{#1}}{q^{#3} _{#1}(#2)}}
\newcommand{\posterior}[2]{\ifthenelse{\equal{#2}{}}{p^\obs _{#1}}{p^\obs _{#1}(#2)}}
\newcommand{\initdistr}[3]{\ifthenelse{\equal{#2}{}}{\chi_{#1}}{\chi_{#1}(#2, #3)}}
% \newcommand{\bwopt}[4]{{\ifthenelse{\equal{#3}{}}{\overleftarrow{m}^{#2} _{#1}}{\overleftarrow{m}^{#2} _{#1}(#3 #4)}}}
\newcommand{\bwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{p^{#2} _{#1}(#4|#3)}}
\newcommand{\bbwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{\underline{p}^{#2} _{#1}(#4|#3)}}
\newcommand{\tbwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{\overline{p}^{#2} _{#1}(#4|#3)}}
\newcommand{\fwopt}[4]{\ifthenelse{\equal{#3}{}}{\overset{{}_{\rightarrow}}{m} ^{#2} _{#1}}{\smash{\overset{{}_{\rightarrow}}{m}}^{#2} _{#1}(#4|#3)}}
\newcommand{\ufilter}[3]{{\ifthenelse{\equal{#3}{}}{\eta^{#2} _{#1}}{\eta^{#2} _{#1}(#3)}}}
\newcommand{\filter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi^{#2} _{#1}(#3)}}}
\newcommand{\noisyfilter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi^{#2} _{#1}(#3)}}}
\newcommand{\noiselessfilter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi _{#1}(#3 | #2)}}}
% \newcommand{\pred}[3]{{\ifthenelse{\equal{#3}{}}{\eta^{#2} _{#1}}{\eta^{#2} _{#1}(#3)}}}
\newcommand{\bfilter}[3]{{\ifthenelse{\equal{#3}{}}{\Phi^{#2} _{#1}}{\Phi^{#2} _{#1}(#3)}}}
\newcommand{\normconstest}[1]{\gamma^N _{#1}}
\newcommand{\Qker}[2]{Q_{#1} ^{#2}}
\newcommand{\lawSMC}[1]{P^N _{#1}}
\newcommand{\lawcSMC}[1]{\mathbf{P}^N _{#1}}

% \newcommand{\anc}[2]{\smash{A^{#1} _{#2}}}
\newcommand{\ianc}[2]{a^{#1} _{#2}}
\newcommand{\iancanc}[2]{b^{#1} _{#2}}
\newcommand{\pot}[3]{\ifthenelse{\equal{#3}{}}{\smash{g^{#2} _{#1}}}{\smash{g^{#2} _{#1}}(#3)}}
\newcommand{\ipot}[3]{\ifthenelse{\equal{#3}{}}{g^{#2} _{#1}}{g^{#2} _{#1}(#3)}}
\newcommand{\iapot}[3]{\ifthenelse{\equal{#3}{}}{\tilde{g}^{#2} _{#1}}{\tilde{g}^{#2} _{#1}(#3)}}
\newcommand{\dubpot}[3]{\ifthenelse{\equal{#3}{}}{G^{#2} _{#1}}{G^{#2} _{#1}(#3)}}
\newcommand{\fwfilter}[1]{\eta^{\ltrmeas} _{#1}}
% \newcommand{\dforward}[1]{\overrightarrow{m}_{#1}}
% \newcommand{\dbackward}[1]{\overleftarrow{m}_{#1}}
% \newcommand{\pot}[1]{g_{#1}}
% \newcommand{\optforward}[1]{\overrightarrow{p _{#1}}}
% \newcommand{\optbackward}[1]{\overleftarrow{p _{#1}}}
\newcommand{\couplepot}[1]{\mathrm{G}_{#1}}
\newcommand{\intvect}[2]{[#1:#2]}
\def\pathmforward{\overrightarrow{\lambda}}
\def\pathmbackward{\overleftarrow{\lambda}}
% \newcommand{\assp}[1]{(\textbf{A}\textbf{#1})}
\newcommand{\clipleb}[3]{\nu^{#2} _{#1}(#3)}
\newcommand{\noisytrans}[3]{\ifthenelse{\equal{#2}{}}{\mathsf{P}_{#1}}{\mathsf{P}_{#1}(#3|#2)}}
% \def\algo{\texttt{MCGdiff}}
\def\ddrm{DDRM}
\def\dps{\texttt{DPS}}
\def\smcdiff{\texttt{SMCdiff}}
\def\ddim{\texttt{DDIM}}
\def\dimg{d}
%\newcommand{\chunk}[3]{{#1}_{#2}^{#3}}
\newcommand{\pchunk}[3]{#1 ^{#2:#3}}
\newcommand{\philter}[2]{\phi_{#1} ^{#2}}
\def\Id{\mathbf{I}}
%\def\Id{I}
\def\ltopstate{\overline{x}}
\def\lbotstate{\underline{x}}
\def\topstate{\smash{\overline{X}}}
\def\bottomstate{\underline{X}}
% \newcommandx\sequence[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2} \}_{#2 \in #3}}}}
\newcommand\projidx[3]{\ifthenelse{\equal{#2}{}}{#1^{\setminus #3}}{#1^{\setminus #3}_{#2}}}
\newcommand\insertidx[3]{#1^{#2, #3}}

\newcommand{\fwpGen}[1]{p^\genparam _{#1}}
\newcommand{\tstep}[1]{{k_{#1}}}
\newcommand{\ustate}[2]{X^{#1} _{#2}}
\newcommand{\lstate}[2]{X^{#1} _{#2}}
\newcommand{\post}[2]{\ifthenelse{\equal{#2}{}}{\pi_{#1}}{\pi_{#1}(#2)}}
% \newcommand{\potn}[2]{\ifthenelse{\equal{#2}{}}{g_{#1}}{g_{#1}(#2)}}
\newcommand{\potn}[2]{\ifthenelse{\equal{#2}{}}{p_{#1}(\obs|\cdot)}{p_{#1}(\obs|#2)}}
\newcommand{\hpotn}[2]{\ifthenelse{\equal{#2}{}}{\hat{g}_{#1}}{\hat{g}_{#1}(#2)}}
\def\tmidfn{\ell}
\newcommand{\tmid}[1]{{\tmidfn_k}}
\newcommandx{\vmu}[1][1=]{\hat\mu^{#1}}
\newcommandx{\vstd}[1][1=]{\hat\sigma^{#1}}
\newcommandx{\vlstd}[1][1=]{\hat\upsilon^{#1}}
\def\vparam{\varphi}
\def\stdq{\sigma_q}
\def\muq{\mu_q}
\newcommand{\std}[1]{\sigma_{#1}}
\newcommand{\var}[1]{\sigma^2 _{#1}}
\newcommand{\mean}[1]{m_{#1}}
\def\vvparam{\psi}
\def\optparam{\param_\star}
%\def\diag{\mathrm{diag}}
\def\diag{\mbox{diag}}

\newcommand{\vub}[1]{\mathcal{L}_{#1}}

%%%%%%%%%%%%%%%%%%%%%
%% mathbf
%\def\bfA{\mathbf{A}}
\def\bfA{A}
\def\bfC{\mathbf{C}}

\newcommand{\tcr}[1]{\textcolor{red}{#1}}

==> sections/gm.tex <==
\section{Gaussian Mixture example}
We consider the following target:
$$
\fwmarg{0}{\bx _0} = \sum_{i = 1} ^M w_i \normpdf(\bx _0; \mu_i, \Id_\dimx) \eqsp.
$$

==> sections/litterature.tex <==
% temporary notation
\newcommand{\indep}{\perp\!\!\!\!\perp}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\note}[1]{\textcolor{blue}{\text{\small{(#1)}}}}


\section{Literature}

\subsection{Diffusion posterior sampling for general noisy inverse problems}
\cite{chung2023diffusion}

\begin{itemize}
    \item Extend the usage of posterior sampling to noisy inverse (linear or nonlinear) problems
        \begin{equation}
            \bm{y} = \bm{\mathcal{A}}(\bm{\bx}_0) + \bm{n}, \quad p(\bm{y} | \bm{\bx}_0) \ \text{the likelihood is known}
            \enspace.
        \end{equation}
        Contributions: solve noisy inverse problems --with Gaussian or Poisson noise-- in the image space (doesn't rely on SVD)
    \item The Core idea of posterior sampling with diffusion models is to leverage the learned prior to perform conditional sampling
    \item The authors define the DDM according to the VP-SDE whose reverse time reads
        \begin{equation}
            \diff \bm{\bx} =  \big[-\frac{\beta(t)}{2} \bm{\bx}_t - \beta(t) \nabla_{\bm{\bx}_t} \log p_t(\bm{\bx}_t) \big] \diff t
                + \sqrt{\beta(t)} \diff \bar{\bm{\omega}}
            \enspace,
        \end{equation}
        where $\bar{\bm{\omega}}$ is Weiner process in reverse-time, where typically, (Stein) score is learned via denoising score matching \cite{vincent2011connection}
        For conditional sampling, they substitute the score by $\nabla_{\bm{\bx}_t} \log p_t(\bm{\bx}_t | \bm{y}) = \nabla_{\bm{\bx}_t} \log p_t(\bm{y} | \bm{\bx}_t) + \nabla_{\bm{\bx}_t} \log (\bm{\bx}_t)$
    \item The authors claim that $p_t(\bm{y} | \bm{\bx}_t)$ is intractable and hence approximate it with
        \begin{equation}
            \begin{aligned}
                p_t(\bm{y} | \bm{\bx}_t)
                    & = \int p_t(\bm{y} | \bm{\bx}_0) p_t(\diff \bm{\bx}_0 | \bm{\bx}_t) \quad \text{\small (Assume that } \bm{y} \indep \bm{\bx}_t \ | \bm{\bx}_0) \\
                    & = \pE _{\bm{\bx}_0 \sim p_t(\diff \bm{\bx}_0 | \bm{\bx}_t)} \big[ p_t(\bm{y} | \bm{\bx}_0) \big]\\
                    & \approx p_t \big( \bm{y} | \pE  [ \bm{\bx}_0 | \bm{\bx _t} ] \big)
            \end{aligned}
            \enspace,
        \end{equation}
        \note{Thanks to Jenson inequality we have  $p_t \big( \bm{y} | \pE  [ \bm{\bx}_0 | \bm{\bx _t} ] \big) \leq  p_t(\bm{y} | \bm{\bx}_t)$}\\
        where they used Tweedie approach
            \begin{equation}
                \pE  [ \bm{\bx}_0 | \bm{\bx _t} ] = \frac{1}{\sqrt{\bar{\alpha}}_t} \big( \bm{\bx}_t + (1 - \bar{\alpha}_t) \nabla_{\bm{\bx}_t} \log p_t(\bm{\bx}_t) \big)
                := \hat{\bm{\bx}}_t
                \enspace,
            \end{equation}
    \item The final form of the conditional gradient in case of $\bm{n}$ begin $\mathcal{N}(0, \sigma^2 \id)$
        \begin{equation}
           \nabla_{\bm{\bx}_t} \log p_t(\bm{y} | \bm{\bx}_t) = -\frac{1}{\sigma^2} \nabla_{\bm{\bx}_t} \norm{y - \bm{\mathcal{A}(\hat{\bm{\bx}_t})}}^2
           \enspace,
        \end{equation}
        \note{I think they make the implicit assumption of $ p_t \big( \bm{y} | \hat{\bm{\bx}}_t \big) \approx p \big( \bm{y} | \hat{\bm{\bx}}_t \big)$}\\
        Afterward, they use the Euler-Maruyama scheme to simulate the reverse SDE
    \item \textbf{Feedback:} Well-written paper with solid experiments; The authors make a good attempts to derive a bound on the approximation error, yet the latter is intractable, intervenes problem specific quantities, and doesn't give insights to control the error or improve the quality of the posterior sampling (aside from using a good denoiser, and the trivial setup of $\sigma \rightarrow \infty$)
\end{itemize}


\subsection{Towards Coherent Image Inpainting Using Denoising Diffusion Implicit Models}
\cite{zhang2023towards}

\begin{itemize}
    \item Image inpainting is to complete an image based on some of its partially revealed parts
    \item Two lines of research of image inpainting using DDM
        \begin{itemize}
            \item supervised: tain a model for a specific inpainting task, train jointly a diffusion and conditional model; Limited by data shortage as it requires a couple of images and labels, being too task-specific and hence hard to extend to other tasks
            \item Unsupervised: performs a conditional sampling on the observation based on a DDM as prior; two major methods blending that consists of replacing the revealed part of intermediate noisy images of their noisy version (leads to incoherences in the final sample) and posterior sampling
        \end{itemize}
    \item The setup choosen by authors is DDIM, the main principle is to cast the inpainting problem as a constraint
        \begin{equation}
            \log p_{\bm{\theta}}(\bm{\bx}_T | \mathcal{C}) \approx -\frac{1}{2} \norm{\bm{\bx}_T}^2 - \frac{1}{2 \zeta_t^2} \norm{\bm{s}_0 - \bm{r}(\bm{f}_{\bm{\theta}}(\bm{\bx}_T))}^2
        \end{equation}
        and use MAP or MCMC estimation \note{$\zeta_t \rightarrow 0$ the constraint becomes a indicator function;} \note{it is a bold statement to say that $\zeta_t$ can be virtually zero}
    \item \textbf{Feedback:} Detailed literature review; The framework is not well refined with many bold statements
\end{itemize}


==> sections/old_method.tex <==
\section{A Gibbs sampler on DDM posterior sampling}
\subsection{Posterior distribution with DDM prior}
In this paper we focus on the task of approximate sampling of a distribution defined as
\begin{equation}
    \label{eq:posterior_def}
   \txts \post{}{\bx} \eqdef \potn{}{\bx} \prior(\bx) / \normconst
  \end{equation}
where $\pot{}{}{}$ is a non-negative likelihood that we assume we can evaluate pointwise, $\prior$ is a prior distribution on which we may have information only through i.i.d. samples and $\normconst \eqdef \int \potn{}{\bx} \prior(\bx) \, \rmd \bx$ is the normalizing constant.
Possible applications include sampling from a posterior distribution, in which case $\potn{}{}$ is the likelihood, or sampling from an unnormalized density.
In the latter, the prior $\prior$ encodes relevant information about the distribution of interest, such as the location of the modes for example or the shape of the tails.

We assume that a DDM has been trained to model \emph{only} the prior distribution $\prior$ and our goal is to devise an algorithm for sampling approximately from $\post{}{}$ while not requiring any further training. This aspect is particularly crucial in applications where one   has access to a \emph{pre-trained} DDM and is interested in performing controlled generation to solve specific tasks defined by different likelihoods $\potn{}{}$.

Consider the joint distribution on $(\rset^\dimx)^{n+1}$ obtained by initializing the forward process with the posterior of interest \eqref{eq:posterior_def}
\begin{equation}
    \label{eq:posterior_forward}
  \post{0:n}{\bx _{0:n}} \eqdef \post{}{\bx _0} \prod_{k = 0}^{n-1} \fwtrans{k+1|k}{\bx _k}{\bx _{k+1}} \eqsp.
\end{equation}
We initiate our approach by replacing the initial problem of sampling from \eqref{eq:posterior_def} with that of sampling from the reverse-time decomposition of \eqref{eq:posterior_forward} which writes
\begin{equation} 
    \label{eq:posterior_backward}
    \post{0:n}{\bx _{0:n}} \eqdef \post{n}{\bx _n} \prod_{k = 0}^{n-1} \pibw{k|k+1}{\bx _{k+1}}{\bx _{k}} \eqsp,
\end{equation}
where for all $k \in \intset{0}{n}$, $\post{k}{\bx _k} \eqdef \int \post{}{\bx _0} \fwtrans{k|0}{\bx _0}{\bx _k} \, \rmd \bx _0$ and
\begin{equation} 
    \label{eq:pibwker}
    \pibw{k|k+1}{\bx _{k+1}}{\bx _{k}} = \post{k}{\bx _k}\fwtrans{k+1|k}{\bx _k}{\bx _{k+1}} \big/ \post{k+1}{\bx _{k+1}} \eqsp, \quad k \in \intset{0}{n-1} \eqsp.
\end{equation}
The decomposition \eqref{eq:posterior_backward} shows that an exact sample from \eqref{eq:posterior_def} is obtained by first sampling $\bX  _n$ from $\post{n}{}$ and then recursively sampling $\bX  _{k} \sim \pibw{k|k+1}{\bX _{k+1}}{\cdot}$ for $k \in \intset{0}{n-1}$. However, the backward transition kernels \eqref{eq:pibwker} prove to be difficult to sample from in practice due to the fact that the likelihoods \eqref{eq:ipot_def} are intractable in general and we cannot leverage a \textsc{DDPM} approximation as by assumption we do not have access to a parametric approximation of the scores $(\nabla \log \post{k}{} )_{k = 1}^{n}$. Instead, we only have access to parametric approximations of the scores $( \nabla \log \fwmarg{k}{} )_{k = 1} ^{n}$ which we leverage using the identity we provide in \Cref{lem:pi_bwker}. First, define for all $k \in \intset{0}{n}$, the likelihoods $(g_k)_{k = 0} ^n$ which satisfy $\potn{0}{} \eqdef \potn{}{}$ and
\begin{equation}
    \label{eq:ipot_def}
    \potn{k}{\bx _k} \eqdef \int \potn{}{\bx _0} \, \rbwker{0|k}{\bx _k}{\bx _0} \, \rmd \bx _0 \eqsp, \quad k \geq 1 \eqsp,
\end{equation}
where $\rbwker{0|k}{\bx _k}{\bx _0} \eqdef \int \prod_{j = 0}^{k-1} \rbwker{j|j+1}{\bx _{j+1}}{\bx _j} \, \rmd \bx _{0:k-1}$.
\begin{lemma} 
    \label{lem:pi_bwker}
    For all $k \in \intset{0}{n-1}$ it holds that
    $$
        \pibw{k|k+1}{\bx _{k+1}}{\bx _k} = \int \fwtrans{k|0, k+1}{\bx _0, \bx _{k+1}}{\bx _k}\eqsp.
    $$
\end{lemma}
The proof is given in \Cref{proof:pi_bwker}. This alternative expression is more appealing as it instead involves the backward transition $\smash{\rbwker{k|k+1}{\bx _{k+1}}{\cdot}}$ of which we can estimate the gradient efficiently using the pre-trained model. The main intractability stems from the likelihood $\potn{k}{\bx _k}$ which is difficult to estimate in practice as it is given by an integral over the complex distribution $\smash{\rbwker{0|k}{\bx _k}{\cdot}}$. The next section is devoted to the development of a variational approach designed to overcome this challenge.

\subsection{The {\sc{VDDPS}} algorithm}
In order to circumvent the intractability of the backward transition $\smash{\seq{\pibw{k|k+1}{}{}}{k=0}{n-1}}$, we propose to replace them with mean-field Gaussian variational approximations $\seq{\vbwker{k|k+1}{}{}[\vparam]}{k=0}{n-1}$ defined by
\begin{equation}
    \vbwker{k|k+1}{\bx _{k+1}}{\bx _k} \eqdef \normpdf\big(\bx _k; \vmu_{k|k+1}, \big(\vstd_{k|k+1}\big)^2 \cdot \Id_\dimx \big) \eqsp,
\end{equation}
where $(\vmu_{k|k+1}, \vstd_{k|k+1}) \in \rset^{\dimx} \times \rset_{> 0}$.
More specifically, to draw one approximate sample from $\post{}{}$ we propose to simulate a Markov chain $(\bX  _{0:n})$ where $\bX _n \sim \normpdf(\zero_\dimx, \Id_\dimx)$ and given $\bX  _{k+1}$, $\bX  _{k}$ is defined as follows. We first optimize an estimate of $(\vparam, \vvparam) \mapsto \vub{k}(\vparam, \vvparam; \bX _{k+1})$, where $\vvparam$ is a second variational parameter, satisfying:
% an upper-bound (defined in the next section) on the backward KL divergence
\begin{equation}
    \label{eq:kl_objective}
    \kldivergence{\vbwker{k|k+1}{\bX  _{k+1}}{\cdot}}{\pibw{k|k+1}{\bX  _{k+1}}{\cdot}} \leq \vub{k}(\vparam, \vvparam; \bX _{k+1}) \eqsp.
\end{equation}
The optimization of this upperbound with respect to both variational parameters yields $\vbwker{k|k+1}{}{}[\vparam_*]$ from which we then sample $\bX _k \sim \vbwker{k|k+1}{\bX _{k+1}}{\cdot}[\vparam_*]$. We focus on defining $\vub{k}$ in the next section.
\paragraph{Variational upper bound.}
Following the \Cref{lem:pi_bwker}, the objective \eqref{eq:kl_objective} writes
\begin{multline*}
    \kldivergence{\vbwker{k|k+1}{\bx _{k+1}}{\cdot}}{\pibw{k|k+1}{\bx _{k+1}}{\cdot}} = - \int \log \potn{k}{\bx _k}\, \vbwker{k|k+1}{\bx _{k+1}}{\bx _k}[\vparam] \, \rmd \bx _k \\
    + \kldivergence{\vbwker{k|k+1}{\bx _{k+1}}{\cdot}}{\rbwker{k|k+1}{\bx _{k+1}}{\cdot}} + \log \potn{k+1}{\bx _{k+1}}\eqsp,
\end{multline*}
for all $\bx _{k+1} \in \rset^\dimx$.
While the second term in the \rhs\ can be readily estimated using the pre-trained DDM as we see next, the first one involves the intractable integral $\potn{k}{}$. To avoid having to evaluate it pointwise we consider the following upperbound.

Let $\bx _k \mapsto \vbwker{0:k-1|k}{\bx _k}{\cdot}[\vvparam]$ be a variational approximation of the conditional joint distribution
\begin{equation}
    \label{eq:pi_0k}
\pibw{0:k-1|k}{\bx _k}{\bx _{0:k-1}} \propto \potn{}{\bx _0} \rbwker{0:k-1|k}{\bx _k}{\bx _{0:k-1}} \eqsp,
\end{equation}
where $\rbwker{0:k-1|k}{\bx _k}{\bx _{0:k-1}} \eqdef \prod_{j = 0}^{k-1} \rbwker{j|j+1}{\bx _{j+1}}{\bx _j}$.
We find by applying Jensen's inequality that
\begin{align*}
    \log \potn{k}{\bx _k} & = \log \int \potn{}{\bx _0} \rbwker{0:k-1|k}{\bx _k}{\bx _{0:k-1}} \, \rmd \bx _{0:k-1} \\
    & \geq \int \log \frac{\potn{}{\bx _0} \rbwker{0:k-1|k}{\bx _k}{\bx _{0:k-1}}}{\vbwker{0:k-1|k}{\bx _k}{\bx _{0:k-1}}[\vvparam]} \vbwker{0:k-1|k}{\bx _k}{\bx _{0:k-1}}[\vvparam] \, \rmd \bx _{0:k-1}
\end{align*}
and hence the following upper bound follows
\begin{multline*}
    - \int \log \,\potn{k}{\bx _{k}}  \vbwker{k|k+1}{\bx _{k+1}}{\bx _k}[\vparam]\, \rmd \bx _k \leq - \int \bigg\{ \int \log \potn{}{\bx _0} \vbwker{0|k}{\bx _k}{\bx _0}[\vvparam] \, \rmd \bx _0 \\
     \hspace{2cm} + \kldivergence{\vbwker{0:k-1|k}{\bx _{k}}{\cdot}[\vvparam]}{\rbwker{0:k-1|k}{\bx _{k}}{\cdot}} \bigg\} \vbwker{k|k+1}{\bx _{k+1}}{\bx _k}[\vparam] \, \rmd \bx _{k} \eqsp.
\end{multline*}
Define for all $\vparam \in \rset^\dimx \times \rset_{>0}$ and $\bx _{k+1} \in \rset^\dimx$
\begin{align}
    \label{eq:vub}
    \vub{k}& (\vparam, \vvparam; \bx _{k+1}) \eqdef
    \kldivergence{\vbwker{k|k+1}{\bx _{k+1}}{\cdot}}{\rbwker{k|k+1}{\bx _{k+1}}{\cdot}} + \log \potn{k+1}{\bx _{k+1}} \\
    & - \pE _{\vbwker{k|k+1}{\bx _{k+1}}{\cdot}} \Big[ \int \log \potn{}{\bx _0} \vbwker{0|k}{\bX _k}{\bx _0}[\vvparam] \, \rmd \bx _0 + \kldivergence{\vbwker{0:k-1|k}{\bX _{k}}{\cdot}[\vvparam]}{\rbwker{0:k-1|k}{\bX _{k}}{\cdot}} \Big] \nonumber
    \eqsp.
\end{align}
Then, it holds that
\begin{equation}
    \label{eq:kl_upper_bound}
\txts \kldivergence{\vbwker{k|k+1}{\bx _{k+1}}{\cdot}}{\pibw{k|k+1}{\bx _{k+1}}{\cdot}} \leq \vub{k}(\vparam, \vvparam; \bx _{k+1}) \eqsp,
\end{equation}
with equality if and only if $\vbwker{0:k-1|k}{\bx _{k}}{}[\vvparam] = \pibw{0:k-1|k}{}{}$. We want to optimize the upper-bound \wrt\ the variational parameters $\vparam$ and $\vvparam$ which in turn requires being able to efficiently estimate expectations under $\vbwker{0:k-1|k}{\bx _{k}}{\cdot}[\vvparam]$. We now present one relevant parameterization.

\paragraph{Parameterization.}
For the variational distribution $\smash{\vbwker{0:k-1|k}{}{}[\vvparam]}$ we consider the parameterization
\begin{equation}
    \label{eq:vx0t}
\txts \vbwker{0:k-1|k}{\bx _{k}}{\bx _{0:k-1}}[\vvparam] \eqdef \vbwker{0|k}{\bx _k}{\bx _0}[\vvparam] \prod_{j = 1}^{k-1} \rbwker{j|0, j+1}{\bx _0, \bx _{j+1}}{\bx _j} \eqsp.
\end{equation}
where $\vbwker{0|k}{\bx _k}{\bx _0}[\vvparam] \eqdef \normpdf(\bx _0; \vmu[\vvparam] _{0|k}(\bx _k), (\vstd[\vvparam] _{0|k})^2 \cdot \Id_\dimx)$. This parameterization is inspired by the fact that \eqref{eq:pi_0k} writes
$$
\txts \pibw{0:k-1|k}{\bx _k}{\bx _{0:k-1}} = \pibw{0|k}{\bx _k}{\bx _0} \prod_{j = 1}^{k-1} \rbwker{j|0, j+1}{\bx _0, \bx _{j+1}}{\bx _j}
$$ and hence $\vbwker{0|k}{\bx _k}{\cdot}$ is understood as a Gaussian approximation of $\pibw{0|k}{\bx _k}{\cdot}$. Using Tweedie's formula, (see XXX), the expectation of $\pibw{0|k}{\bx _k}{\cdot}$ is given approximately by $\smash{\predxs{k}(\bx _k) + (1 - \acp{k}) \nabla_{\bx _k} \log \potn{k}{\bx _k} \big/ \sqrt{\acp{k}}}$ which prompts us to use the following parameterization for the mean of $\vbwker{0|k}{\bx _k}{\cdot}[\vvparam]$:
\begin{equation}
    \vmu[\vvparam] _{0|k}(\bx _k) \eqdef \big(\predxs{k}(\bx _k) + \vmu[\vvparam]_k\big) \big/ 2 \eqsp, \quad \vmu[\vvparam]_k \in \rset^\dimx \eqsp.
\end{equation}
The $\frac{1}{2}$ factor allows us to use $\predxs{k}(\bx _k)$ as initialization for $\vmu[\vvparam]_k$ so that $\vmu[\vvparam] _{0|k}(\bx _k)$ is equal to $\predxs{k}(\bx _k)$ initially.
As a result of this parameterization, the optimization of the upper-bound over $\vvparam$ boils down to optimizing $(\vmu[\vvparam] _{0|k}, \vstd[\vvparam] _{0|k})$ over $\rset^\dimx \times \rset _{> 0}$. We can now provide a gradient estimator for $\vub{k}$.

\paragraph{Gradient estimator.}
It follows from the parameterization \eqref{eq:vx0t} that the gradient \wrt\ $(\vparam, \vvparam)$ of the KL divergence term between the conditional joint distributions in \eqref{eq:vub} writes
\begin{align*}
\nabla_{\vparam, \vvparam} \, & \pE _{\vbwker{k|k+1}{\bx _{k+1}}{}} \left[ \kldivergence{\vbwker{0:k-1|k}{\bX _{k}}{\cdot}[\vvparam]}{\rbwker{0:k-1|k}{\bX _{k}}{\cdot}} \right] \\
& = \sum_{j = 0} ^{k-1} \pE \bigg[ - \big(\nabla_{\vparam, \vvparam} \bX ^{\vparam, \vvparam} _{j|0, j+1} \big)^\intercal \nabla_{\bx _j} \log \fwmarg{j}{\bX ^{\vparam, \vvparam} _{j|0, j+1}} - \nabla_{\vparam, \vvparam} \log \fwtrans{j+1|j}{\bX ^{\vparam, \vvparam} _{j|0, j+1}}{\bX ^{\vparam, \vvparam} _{j+1|0, k}}\\
& + \big(\nabla_{\vparam, \vvparam} \bX ^{\vparam, \vvparam} _{j+1 |0, k} \big)^\intercal \nabla_{\bx _{j+1}} \log \fwmarg{j+1}{\bX ^{\vparam, \vvparam} _{j+1 |0, k}}\bigg]
\end{align*}
\begin{lemma}
    For all $(\vparam, \vvparam)$ and $\bx _{k+1} \in \rset^\dimx$, it holds that
    \begin{multline}
        \vub{k}(\vparam, \vvparam; \bx _{k+1}) = \frac{\| \vmu[\vparam] _{k|k+1} - \muDDIM{k|k+1} \|^2 + \dimx (\vstd[\vparam] _{k|k+1})^2 }{2 \sigma^2 _{k|k+1}} - \dimx \log \vstd[\vparam] _{k|k+1} + \frac{\dimx}{2} \log \big[ \frac{(1 - \acp{k})(\vstd[\vvparam]_0)^2}{1 - \acp{k} + \acp{k} (\vstd[\vvparam]_{0})^2} \big]\\
        + \pE_{\vbwker{0, k|k+1}{\bx _{k+1}}{\cdot}[\vparam, \vvparam]} \bigg[
             \log \potn{}{\bX _0} +  \sum_{j = 1}^{k-1} w_{j} \pE_{\vbwker{j|0, k}{\bX _0, \bX _k}{\cdot}[\vvparam]} \big[ \| \bX _0 - \predxs{j}(\bX _j) \|^2 \big]
        \bigg] + C_{k|k+1} \eqsp, \nonumber
    \end{multline}
    where
\end{lemma}
\begin{multline*}
    \kldivergence{\vbwker{0:k-1|k}{\bX _{k}}{\cdot}[\vvparam]}{\abwker{0:k-1|k}{\bX _{k}}{\cdot}} \\
    = \sum_{j = 1}^{k-1} w_j \pE_{\vbwker{0|k}{\bX _k}{\cdot}[\vvparam] \otimes \normpdf(\zero_\dimx, \Id_\dimx)} \left[ \| \bX _0 - \predxs{j}(\sqrt{\acp{j}} \bX _0 + \sqrt{1 - \acp{j}} \bZ) \|^2 \right] \eqsp,
\end{multline*}
where $w_j = $.

\subsection{Application to sampling from an unnormalized density}
% \paragraph{Jacobian-free approximation.} \begin{align*}
%     \vmu[\vvparam] _{0|k}(\bx _k) & \eqdef \big( (1 - \acp{k}) \vmu[\vvparam] _0 + \sqrt{\acp{k}} (\vstd[\vvparam] _0)^2 \bx _k \big) \big/ (1 - \acp{k} + \acp{k} (\vstd[\vvparam]_{0})^2)  \eqsp, \\
%     \vstd[\vvparam]_{0|k} & \eqdef \sqrt{1 - \acp{k}} \vstd[\vvparam]_0 \big/ \sqrt{ 1 - \acp{k} + \acp{k} (\vstd[\vvparam]_{0})^2 } \eqsp.
% \end{align*}
% with $(\vmu[\vvparam] _{0}, \vstd[\vvparam] _0) \in \rset^\dimx \times \rset_{> 0}$ being the parameters over which we perform the optimization. This parameterization assumes implicitely a Gaussian variational approximation for the posterior of interest $\post{0}{}$. Indeed, letting $\vbwker{0}{}{}[\vvparam](\bx _0) \eqdef \normpdf(\bx _0; \vmu[\vvparam]_0, (\vstd[\vvparam] _0)^2 \Id_\dimx)$,  we have that $\smash{\vbwker{0|k}{\bx _k}{\bx _0}[\vvparam] \propto \vbwker{0}{}{}[\vvparam](\bx _0) \fwtrans{k|0}{\bx _0}{\bx _k}} \eqsp.$

